The Effect of Sensor Fusion on Data-Driven Learning of Koopman Operators

Dictionary methods for system identification typically rely on one set of measurements to learn governing dynamics of a system. In this paper, we investigate how fusion of output measurements with state measurements affects the dictionary selection process in Koopman operator learning problems. While prior methods use dynamical conjugacy to show a direct link between Koopman eigenfunctions in two distinct data spaces (measurement channels), we explore the specific case where output measurements are nonlinear, non-invertible functions of the system state. This setup reflects the measurement constraints of many classes of physical systems, e.g., biological measurement data, where one type of measurement does not directly transform to another. We propose output constrained Koopman operators (OC-KOs) as a new framework to fuse two measurement sets. We show that OC-KOs are effective for sensor fusion by proving that when learning a Koopman operator, output measurement functions serve to constrain the space of potential Koopman observables and their eigenfunctions. Further, low-dimensional output measurements can be embedded to inform selection of Koopman dictionary functions for high-dimensional models. We propose two algorithms to identify OC-KO representations directly from data: a direct optimization method that uses state and output data simultaneously and a sequential optimization method. We prove a theorem to show that the solution spaces of the two optimization problems are equivalent. We illustrate these findings with a theoretical example and two numerical simulations.

==> Abstract_and_Intoduction/Introduction_WhatHappensInTheRestOfThePaper.tex <==
The paper is organized as follows: In section \ref{sec: Basic Idea} we introduce the problem of identifying OC-KOs. In section \ref{sec: math prelims}, we briefly discuss the Koopman operator theory and the necessary DMD algorithms. In section \ref{sec: oc- Koopman}, we discuss the theory of output constrained Koopman operators. We describe the OC-deepDMD algorithm in section \ref{sec: oc-deepDMD} and the numerical examples in section \ref{sec: Simulation Results} to show its performance, limitations and a method to  overcome it. 

\begin{comment}
In section \ref{sec: oc-deepDMD}, we describe the OC-deepDMD algorithm as a method to identify these models. In section \ref{sec: Simulation Results}, we consider three examples in increasing orders of complexity to show that the OC-deepDMD algorithm finds Koopman operator representations that capture the state and output dynamics accurately with excellent multistep prediction capability. We use an oscillator example to bring out the limitations of the algorithm and discuss a method to overcome it.  
\end{comment}

\begin{comment}
The paper is organized as follows: In section \ref{sec: Basic Idea} we introduce the problem of identifying a high dimensional linear state space model of a nonlinear system in which both the states and the outputs are measured and the optimization problem that corresponds to it. In section \ref{sec: math prelims}, we briefly discuss the Koopman operator theory and the necessary DMD algorithms. In section \ref{sec: oc- Koopman}, we reason that the existing Koopman framework is inadequate to accommodate for both state and output measurements and hence, introduce the output constrained Koopman operator in which only a subset of the observables of the Koopman operator are constrained on the output. We show that an output constrained Koopman operator representation exists such that the true state dynamics can be recovered under certain conditions on the system dynamics. In section \ref{sec: oc-deepDMD}, we discuss the output constrained deep DMD (oc-deepDMD) algorithm as an extension of deep DMD algorithm from \cite{yeung2019learning} to include the output constraints. We discuss two different formulations of the oc-deepDMD problem with one formulation rendering a relatively sparse solution than the other. We discuss that a transformation of variables is necessary for the neural network to learn a good model and show how the transformation affects the Koopman operator representation. In section \ref{sec: Simulation Results}, we consider three examples in increasing orders of complexity to show that both oc-deepDMD algorithms find Koopman operator representations that capture the state and output dynamics accurately with excellent multistep prediction capability. We use an oscillator example to bring out the limitations of the algorithm and discuss how to overcome it for the oscillator example. 
\end{comment}

==> Abstract_and_Intoduction/intro_7.tex <==
Definition of sensor fusion, list all the references in the literature at large

Categorical description of the 3 classes of sensor fusion algorithms, strengths & limitations  (--> unwieldy models in the model ID space)

KO models are both analytical and data-driven, allows for discovery of model class directly from state and output measurements.   What is KO theory? 

But sensor fusion has not been explored in KO modeling. 

Sensor fusion matters in a recent problem we have looked at  in biology.  This sensor fusion problem is distinct from standard sensor fusion in autonomy and ... because ... 


Thus, in this paper, we look at KO approaches for sensor fusion.  We study the effects of sensor fusion on KO observable subspace geometry...  Our contributions are as follows: 1) ... 2) ... 3) ... 







Sensor fusion is the art of integrating multiple sensor signals to gather information or increase knowledge about an observed, physical system.   Sensor fusion methods are useful when the information gained from multiple sensor sources exceeds the information that can be derived from an isolated sensor channel.  Typical sensor fusion problems center on estimating the dynamical state \cite{StateEstimationSensorFusionPapers} or the model parameters for a physical system of interest \cite{SensorFusionInformationGainPapers}.      

2.O:There are three broad classes of sensor fusion algorithms: 1) .... 2) ... 3).  In competitive. ...  




2.E (1) :  Sensor fusion algorithms that act to estimate model dynamics typically result in nonlinear input-output or state-space models that are unwieldy for analysis and control.  -->  


There is a need for sensor fusion algorithms that result in analytically nice representations.  One such field is KO models.  




There are many approaches for identifying dynamical system models for physical systems with nonlinear behavior.  In particular, a broad class of methods considers developing phenomenological models that describe behavioral or dynamical relationships between measured input and output variables, with no implicit representation of state space dynamics.  Examples of these methods include Volterra series models \cite{cheng2017volterra,stegmayer2004towards, nelles3nonlinear}, Hammerstein-Weiner models \cite{bai2019recursive}, dictionary-based models of nonlinear dynamics \cite{brunton2016discovering, pan2015sparse}.  These models develop coarse grained representations of system dynamics, wholly in terms of directly measured quantities.  

An alternative approach is to 

If the measurements can represent the full state of the system, KORs can capture the governing dynamics from the data \cite{brunton2016discovering,rowley2009spectral,taira2017modal} by identifying high dimensional linear models of the nonlinear system, enabling the usage of tools from linear systems theory \cite{budivsic2012applied, korda2018linear} to study them. 
Due to this, KORs gained a lot of traction in various applications like fluids \cite{arbabi2017study,rowley2010reduced,bagheri2013koopman}, power systems \cite{hernandez2018nonlinear,susuki2016applied,korda2018power}, robotics \cite{gutow2020koopman,bruder2019nonlinear,castano2020control}, etc. But what if we have measurements of both states and outputs?\\

 Sensor fusion is the art of combining measurements from multiple sensors to provide better information about the system than that would be possible with individual sensors \cite{bachmann2011multi}. In inertial navigation systems for general aviation, sensors like the inertial mass unit (IMU) \cite{hasan2009review}, global navigation satellite system \cite{hansen2017nonlinear} and radio frequency beacons \cite{shankar2019finite} have been used in various combinations to estimate its position and orientation. Transportation management centers aim to monitor and control traffic by fusing the measurements from route trackers, Bluetooth, loop detectors to estimate traffic speed and travel time\cite{bachmann2011multi}. Sensor fusion architectures have been implemented in the above systems to extract accurate information about the features of interest and their relationship with the measured variables is established.\\ 

In biological systems, insights about the system have been gained using datasets from individual instruments. While some data like transcriptomics \cite{wang2009rna} and proteomics \cite{aebersold2003mass} investigate the gene and protein activity respectively within the cells, other instruments like microscopes\cite{lefman2004three}, plate readers\cite{meyers2018direct} and flow cytometers \cite{gant1993application} examine the morphological traits like fluorescence and population growth outside the cell. There are no models to map the external features to the internal activity of the cell. For such systems where the relationship between sensor measurements and the states of interest is not available, it is not possible to obtain a holistic picture of the model. Moreover, sensor fusion methods to use outputs to get accurate information about the states cannot be done. In this paper, we attempt to leverage the power of Koopman operators to identify sensor fusion models and study the effects of sensor fusion on learning the KORs. \\


We consider the simpler case of an autonomous nonlinear system (no inputs) with a direct full state measurement as well as measurements from other sensors that have a nonlinearly related to the state. How do we identify Koopman operator representations that fuse the two measurements? The most prevalent method to identify Kooopman operators in general is by the dynamic mode decomposition (DMD) algorithm \cite{schmid2010dynamic} and its variants \cite{askham2018variable,kaneko2019convolutional,azencot2019consistent,manohar2019optimized,sinha2019computation,yeung2019learning,hasnain2019data}. The basic idea is to collect all the measured variables and form a concatenated state. This is then lifted to a high dimensional space where the approximate linear dynamics of the system are identified. The inter-dependency between the states and outputs, given by the output equations, are captured intrinsically in the model. As a result, these models are valid in the space of the concatenated states, but only in the region where the output equations hold true. But we do not learn them and hence, lose information on the validity of the model. Moreover, there is a possibility of identifying models where the outputs substitute the observable states of the system in which case, we lose information about the governing state dynamics. This model cannot be used for sensor fusion as the outputs can no longer inform the states. To overcome these issues, we propose the usage of Koopman operator models with linear representations of the output equations which capture the output equations explicitly. These models have been used for theoretical study in \cite{yeung2018koopmanGramian,surana2016koopman,surana2016linear,mamakoukas2020learning,hasnain2019optimalReporterPlacement,mesbahi2021nonlinear} with the assumption that the outputs lie in the span of the lifting functions. We prove that for these model structures, the output equations constrain the lifting functions of the Koopman operator. Hence, we term them as output constrained Koopman operators (OC-KO).\\


 We theoretically show that state-inclusive OC-KO do exist is the system dynamics are analytic. To learn the OC-KO models from data, we pose a new class of DMD algorithms that learn Koopman operators on the state variables with the constraint that the output equation is linear. We term them as the output constrained DMD (OC-DMD) algorithm. We show that the problem can be formulated in two ways- the direct OC-DMD approach where the state and output equations are learnt concurrently and the sequential OC-DMD approach where the two models are learnt separately and fused after. The difference between the two lies in the modal decomposition. The sequential one can clearly draw a distinction between the modes that appeared due to the dynamics and the output which the direct one cannot do. The sequential one yields relatively sparse solutions but the problem is more complex to solve. In practice, we implement the OC-DMD algorithm using the deep DMD \cite{yeung2019learning} approach. Deep DMD algorithm identifies Koopman operators with good multistep predictive capabilities by learning neural network representations of lifting functions in an unconstrained optimization setting. We impose the linear output constraint on the deep DMD algorithm to find the OC-KO models. We call it the output constrained deep DMD (OC-deepDMD) algorithm. We evaluate the performance of the algorithms on three simulation examples of nonlinear systems with nonlinear output in increasing orders of complexity - 1) system with a theoretical finite Koopman operator representation, 2) system without a finite representation but with one equilibrium point and 3) system with a limit cycle. We compare them with either the analytical solution or the nonlinear state space representation identified by neural networks to bring out their advantages and the limitations.\\
 
 
 \begin{comment}
\textcolor{red}{\textbf{Previous iteration:}
Identifying models or governing equations to describe the dynamics  of real-world  physical  systems  can  be  challenging, especially when they exhibit nonlinear behavior. The most commonly used nonlinear system identification model structures that capture the relationship between the input and output data are Volterra series models which are nonlinear finite impulse response models \cite{schetzen1980volterra}, boxed structured models like that of Hammerstein \cite{billings1979non} and Weiner \cite{guo2003identification} which separate the linear and the nonlinear components and the nonlinear autoregeressive model with exogenous inputs (NARX model) which assumes the current output is a function of finite past inputs and outputs \cite{schoukens2009wiener}. The nonlinearities were initially represented by polynomial kernel functions because of their universal function approximation properties.
The polynomial based models do not scale well to a general class of nonlinear systems as, when the deviation of the system from linear regime increases, the number of regressors required to capture the nonlinearities increase exponentially \cite{nelles3nonlinear}. This was rectified by the advent of neural network representations that parsimoniously capture the kernel functions by minimizing the error in the input-output model \cite{boussaada2018nonlinear,stegmayer2004towards,wang2008hammerstein}. These models function as good multistep predictors but are not in a usable form for model based control. Hence, the nonlinear state space models which map the input to the output via a set of hidden variables called the states became prominent. These states represent information about the system and the control theory of these systems is developed in \cite{nijmeijer1990nonlinear,khalil2014nonlinear}. Weiner-Hammerstein models and NARX models have been reformulated as nonlinear state space models in \cite{ase2009state} and \cite{vassiljeva2010state} respectively. Independent methods to identify nonlinear state space models have been proposed in \cite{schon2011system,paduart2010identification} and these models have been used in model predictive control (MPC) applications \cite{abouelazayem2019adaptive}.

Nonlinear MPC optimization problems are difficult to solve and are computationally complex as compared to linear systems. The models discussed up to this point do not assume any prior knowledge of the system and are built purely from data and hence, are referred to as the black box models. The black box state space models do not encapsulate the physics of the system as the states cannot be identified uniquely without measuring them. The Koopman operators \cite{mezic2005spectral} which assume the measured output to be the state of the system are infinite dimensional linear state space models of finite dimensional nonlinear systems. Since they make a prior assumption that the measured output is the state of the system, they can be classified as grey-box models according to \cite{bohlin2006practical}. Finite representations of these Koopman operators are identified using the dynamic mode decomposition (DMD) algorithm \cite{schmid2010dynamic}.The Koopman operator framework has been developed for continuous time systems \cite{budivsic2012applied}, discrete time systems \cite{williams2015data,rowley2009spectral} and input-controlled systems \cite{proctor2016dynamic,williams2016extending}. Observability and controllability concepts have been established by constructing a Koopman gramian \cite{yeung2018koopmanGramian} and MPC using Koopman models is shown in \cite{korda2018linear}.

}


 Consider the situation where we have two sets of measurements with one corresponding to the state and the other to the output. Can we identify a grey box linear state space model using Koopman operator theory? In this paper, we develop a variant of the DMD algorithm that is suited to identify high dimensional linear state space models of nonlinear systems by combining both state and output measurements. Since Koopman models are traditionally obtained by constructing a nonlinear transformation of the state, we begin by showing that the addition of the output equation constrains this transformation. We consider the deep DMD algorithm in  \cite{yeung2019learning} where the nonlinear transformation of the state is obtained by feed-forward neural networks such that the original states are included. We extend this algorithm to include the output measurements and identify a linear output equation in addition to the linear state equation. We term this algorithm as the output constrained deep DMD (OC-deepDMD) algorithm. 

 OC-deepDMD identified Koopman models play an important role in  observability and controllability analysis. In biological systems, mapping the genetic activity in the cells to an observed phenotype is commonly done. Some examples include identifying the genes that regulate a metabolic pathway \cite{atsumi2008metabolic,youngquist2013production,dal2011identification} and genes associated with traits like age at menarche, body mass index, breast cancer, etc. \cite{mancuso2017integrating,nacht1999combining,guo2020integrated,kellis2003sequencing}. In these systems, if we obtain both the genotype and phenotype data as the state and output data, an output constrained Koopman operator representation can be identified. Observability analysis of this model to obtain the subset of genes that manifest as the phenotype, controllability analysis to design actuators that can control the phenotype and MPC policies to get a desired phenotypic characteristic are some ways in which this model can be used. OC-deepDMD identified Koopman models are also useful in sensor fusion applications where multiple sensor information are fused to obtain a better estimate of the state. In aerospace applications \cite{shankar2019finite}, where we have direct measurements of the state as well as other output measurements to improve the accuracy of the state estimate, this model provides a good platform to do sensor fusion.
\end{comment}
\begin{comment}
\textcolor{red}{\textbf{[RESOLVE]}: Need to redo this paragraph}
To discover the class of nonlinearities that govern the system dynamics, we integrate the framework of deep learning and the theory of Koopman operator, to present a novel algorithm called output-constrained deep dynamic mode decomposition or (OC-deepDMD).   The algorithm presents a significant extension and revision of the {\it state-dependent} framework presented in deep dynamic mode decomposition \cite{yeung2019learning}, as it revises the flow of state and output variables to incorporate output-function constraints, propagated through multi-step Koopman operator predictions.   The algorithm  presents a novel perspective for the problem of output-constrained Koopman learning, as a complement to the problem of learning open-loop Koopman operators using deep neural networks, machine learning or dictionary approaches \cite{proctor2016dynamic,proctor2018generalizing,yeung2018koopmanGramian,williams2015data,williams2016extending,mezic2005spectral,lorsch2018,takeishi2017learning}.    As the output function of a physical system is the most manifest physical property of a dynamic system,  OC-deepDMD represents one of the first efforts into performing physics-informed Koopman operator deep learning \cite{stinis2019}.   The algorithm also represents a first attempt at using the Koopman operator method to address problems in sensor fusion, though notable efforts to construct Koopman operator representations in a wide range of physical systems (though not simultaneously) are abundant in the literature \cite{you2018deep,arbabi2019data,arbabi2017ergodic}.
\end{comment}

==> Abstract_and_Intoduction/intro_8_extra.tex <==





%The fusion methods can be categorized based on how the sensors capture the features of the system \cite{mitchell2007multi,durrant1990sensor}. Sensors are said to have a complementary, competitive or cooperative configuration if the measured variables are independent, equal or have some inter-dependence respectively. Sensors have a complementary configuration if they all measure unique features of the system and their direct amalgamation yields more information about the system. thermometers measuring temperatures at different geographical locations \cite{bachmann2011multi} is an example. In competitive configuration, all sensors independently measure the same feature. They are handled by state estimation algorithms like Bayesian filtering \cite{mitchell2007multi}. A good example is in the INS for general aviation which uses myriad sensors to independently estimate its position and orientation \cite{sasiadek2002sensor,hasan2009review,hansen2017nonlinear,shankar2019finite,rigatos2007extended,rigatos2010extended,yazdkhasti2018multi}. Sensor fusion improves the accuracy of the features and is robust to sensor failures. Cooperative sensor fusion is where multiple sensors are jointly used to estimate a feature. This is done using the underlying physics of the system that map the features to the output. An example is seen in the estimation of kinematic and kinetic features of the gait cycle \cite{qiu2018mems,cattin2001sensor, kong2009gait}. An array of sensors can have multiple configurations.




% IMUs from various locations, force plates, CCD-camera, air pressure sensors to estimate various kinematic and kinetic features of the gait cycles using physics based models  \cite{qiu2018mems,cattin2001sensor, kong2009gait}. An array of sensors can have multiple configurations. If each sensor measures a unique feature, the sensors have a complementary configuration. The data can be directly concatenated to give more information about the system. Thermometers measuring temperatures at different geographical locations \cite{bachmann2011multi} is an example. Competitive sensor configuration is when all sensors independently measure the same feature. They are handled by state estimation algorithms like Bayesian filtering \cite{mitchell2007multi}. They are handled by algorithms like Bayesian filtering \cite{mitchell2007multi} which include the well-known Kalman filter and its variants to provide more accurate feature estimates from the redundant information and are robust to sensor failure. In the event that each sensor measures the same feature, there is redundancy of information and is called the competitive sensor configuration. They are handled by algorithms like Bayesian filtering \cite{mitchell2007multi} which include the well known Kalman filter and its variants to provide more accurate feature estimates from the redundant information and are robust to sensor failure. This is very common in systems like the inertial navigation systems (INS) used in automotives and general aviation, where various sensors like the inertial mass unit (IMU) \cite{hasan2009review}, global navigation satellite system \cite{hansen2017nonlinear} and radio frequency beacons \cite{shankar2019finite} compute the position and orientation of the INS independently and are fused to provide joint accurate estimates \cite{sasiadek2002sensor,hasan2009review,hansen2017nonlinear,shankar2019finite,rigatos2007extended,rigatos2010extended,yazdkhasti2018multi}. The other situation is where all sensor measurements are required to estimate the features. This encompasses the cooperative sensor configuration and is extremely sensitive to sensor failures. An example is seen in the gait cycle analysis where IMUs from various locations, force plates, CCD-camera, air pressure sensors to estimate various kinematic and kinetic features of the gait cycles using physics based models  \cite{qiu2018mems,cattin2001sensor, kong2009gait}. An array of sensors can have multiple configurations.
% Some extra good points

% To elucidate the various sensor configurations, we consider the problem of feature extraction from data.



 In such cases where physics-based models are absent or incomplete, it is imperative to use data and capture the relationship between the variables of interest. 
 
In biological systems, insights about the system have been gained using datasets from individual instruments. While some data like transcriptomics \cite{wang2009rna} and proteomics \cite{aebersold2003mass} investigate the gene and protein activity respectively within the cells, other instruments like microscopes\cite{lefman2004three}, plate readers\cite{meyers2018direct} and flow cytometers \cite{gant1993application} examine the morphological traits like fluorescence and population growth outside the cell. There are no models to map the external features to the internal activity of the cell. For such systems where the relationship between sensor measurements and the states of interest is not available, it is not possible to obtain a holistic picture of the model. Moreover, sensor fusion methods to use outputs to get accurate information about the states cannot be done. In this paper, we attempt to leverage the power of Koopman operators to identify sensor fusion models and study the effects of sensor fusion on learning the KORs.

The appropriate sensor fusion method can be used to extract features from data when the sensor configuration can be represented by physical relations. The required models that map the sensors to the features of interest may not always be available. In such cases, the features need to be measured and the models are to be identified. Model identification is another instance of cooperative sensor fusion as we bring in information from different interdependent sensors to gain more information about the system. This includes the dynamical models which fuse the data of a single variable across time, the static models which fuse multivariable data independent of time and the combination of both. Static models are seen in condition monitoring examples like gait cycle analysis and bioreactors where models are identified to use data from multiple sensors to predict the stage of the gait cycle or the reaction respectively. Dynamic models  


One of the common problems is to identify models that map the data to the required features and use the features to estimate the stage of the process. In gait cycle analysis and bioreactors, the measured parameters are mapped to the required features and a classifier model is learnt to predict the stage of the gait cycle or the reaction. Such models can be used to monitor the stage of the bioreactor or develop hybrid control algorithms for the various stages of the gait cycle. 


==> Abstract_and_Intoduction/intro_skeleton.tex <==
Broad Idea: Paragraphs 1 and 2 indicate why we wanna do Koopman + sensor fusion. Paragraphs 3 and 4 indicate how are we gonna do it. After talk about what we wanna do. \\
What is missing right now- Is there any literature for sensor fusion + model identification? Answer is all multivariate system identification- what purpose do they serve

\textbf{A point to add later:} We explore the synergy or the necessity of synergy between the output functions and the lifting functions. 

\newpage
.
\newpage
\textcolor{blue}{
\textbf{Ideas of Paragraph 1: Sensor fusion}
\begin{itemize}
    \item \textbf{Why} sensor fusion? - Intro line - wow factor 
    \item  \textbf{How} is sensor fusion done? - Generic definition of sensor fusion
    \item  \textbf{What} has been done in sensor fusion?
    \item \textbf{Important Notes}
    \begin{itemize}
        \item Our focus is not on sensor fusion
        \item The focus is on the Koopman operator learning problem. 
        \item The motivation stems from the sensor fusion problem
        \item The more time we spend dealing with sensor fusion, the more we are setting the stage for Koopman operator used in sensor fusion and we have no relevance to that problem in this paper
    \end{itemize}
\end{itemize}
}
In this paper, we focus on identifying models 

 Classifier models are built to map these features to the phases of the gait cycle so as to implement appropriate control algorithms for each phase \cite{meng2010emg,ziegler2018classification}. In the absence of physics-based models that map the measurements to the features, the features are measured as well and a model mapping the measurements to the features is identified. A good example is in the bioprocessor \cite{cimander2002sensor} where a combination of an electronic nose sensor and near-infrared spectrometer to develop models that map the measured outputs to the process states like the concentrations...
A similar approach was adopted in the gait cycle system as well in \cite{zhao2019adaptive} where neural networks were used to extract the features from data and hidden markov models were used to map the features to the phase of the gait cycle. 



\cite{ulloa2013determination} - a biology example to distinguish between the honey. 

\cite{zhao2019adaptive} - model identification (HMM) for identifying the phase of the system from the features identified from the . 6 gait events - heel strike, foot flat, mid-stance, heel off, toe off, and mid-swing. NN to extract features from data and a HMM to classify the phase

Linear system identification for control - \cite{garcia2004sensor,artemiadis2010emg}. 

\begin{comment}

Sensor fusion has been successfully deployed in inertial navigation systems (INS), human gait, traffic systems, etc. as the necessary relationships between the measured variables and the features of interest have been established. One of the obstacles of sensor fusion in biological systems is the complexity of the nonlinear behavior. 

Sensor fusion in biological systems and chemical systems have been saturated due to







The key advantage of this approach is that Koopman operators embed the nonlinear system dynamics in a high dimensional linear spaces and allow the usage of linear systems tools to access nonlinear systems. Koopman operators are traditionally learnt by considering the mea

ution of Koopman operator based models integrate sensor data to learn the underlying dynamics, aid in state estimation and  makes it a promising approach for sensor fusion. 





Koopman operators represent the dynamics of nonlinear systems in high dimensional linear systems. The dynamic mode 


Koopman operator theory has evolved as an effective way to identify the underlying dynamics by fusing the state measurements. 


evolved as an effective method of identifying the underlying dynamics from data. Koopman operators 






Sensor fusion has played a pivotal role in many applications. In human gait, senor fusion methods have been deployed to study the dynamics \cite{meng2010emg,ziegler2018classification,zhao2019adaptive, horst2019explaining,alharthi2019deep}, detect anomalies \cite{ajay2018pervasive, paragliola2018gait, bonetto2019seq2seq} and control prosthetics \cite{grimmer2016powered,guo2010study,hoover2012stair,au2005emg,huang2011continuous,zhang2019sensor}. Numerous sensors have been used in inertial navigation systems (INS) to aid in accurate state estimation \cite{sasiadek2002sensor,hasan2009review,hansen2017nonlinear,shankar2019finite,rigatos2007extended,rigatos2010extended,yazdkhasti2018multi} and autonomous vehicle control \cite{hegrenaes2007towards}. In bioreactors, fusion methods have been used to learn the relationship between the sensor data to monitor and control the reaction stages. Sensor fusion has also made its mark in other domains like in manufacturing systems to optimize throughput, in traffic systems to minimize congestion and in structural systems to monitor fatigue. 

Sensor fusion has played a pivotal role in many applications like to analyze cycles \cite{meng2010emg,ziegler2018classification,zhao2019adaptive, horst2019explaining,alharthi2019deep}, detect anomalies \cite{ajay2018pervasive, paragliola2018gait, bonetto2019seq2seq} and control prosthetics \cite{grimmer2016powered,guo2010study,hoover2012stair,au2005emg,huang2011continuous,zhang2019sensor} in human gait systems, to optimize the throughput \cite{shi2018using,pratama2019metacognitive,dou2020unsupervised,kuntouglu2021investigation,bleakie2013feature,gu2017product,he2017integrated} and quality \cite{lin2021metal,francis2019deep,shevchik2017acoustic} of manufacturing processes and to increase the accuracy of inertial navigation systems (INS) \cite{sasiadek2002sensor,hasan2009review,hansen2017nonlinear,shankar2019finite,rigatos2007extended,rigatos2010extended,yazdkhasti2018multi}. 

In human gait analysis, sensor fusion is used to study the gait dynamics  \cite{meng2010emg,ziegler2018classification,zhao2019adaptive, horst2019explaining,alharthi2019deep}, identify gait anomalies like Parkinson's disease \cite{ajay2018pervasive, paragliola2018gait, bonetto2019seq2seq},  control prosthetics \cite{grimmer2016powered,guo2010study,hoover2012stair,au2005emg,huang2011continuous,zhang2019sensor}, etc. Sensor fusion is used in manufacturing industries to monitor tool wear \cite{shi2018using,pratama2019metacognitive,dou2020unsupervised,kuntouglu2021investigation,bleakie2013feature}, assess product quality \cite{lin2021metal,francis2019deep,shevchik2017acoustic} and predict maintenance schedules \cite{gu2017product,he2017integrated} to optimize the throughput and quality of the manufacturing processes. In navigation systems, it is used to estimate features like position and orientation with utmost accuracy and ensure that the estimation process is robust to sensor failures \cite{sasiadek2002sensor,hasan2009review,hansen2017nonlinear,shankar2019finite,rigatos2007extended,rigatos2010extended,yazdkhasti2018multi}. Sensor fusion has also made its mark in other areas like bioreactors \cite{cimander2002sensor}, structural systems \cite{}, traffic systems \cite{} and healthcare \cite{}. 
\end{comment}

\textcolor{ForestGreen}{\textbf{Why is sensor fusion useful?}
\begin{itemize}
    \item Integrating the data to provide a complete picture of the system. Why is this useful?
    \begin{itemize}
        \item Maybe understand the underlying system better
        \item 
    \end{itemize}
    \item Mapping the data to the key features of the system. Why is this useful?
    \begin{itemize}
        \item Condition monitoring - Why is this useful?
        \begin{itemize}
            \item Prevent catastrophic failure, maintenance scheduling - structural monitoring, 
            \item Health monitoring - identify cow mastitis, rehabilitation
            \item quality control - 
        \end{itemize}
        \item If features are the states - Indicate where the system is at. Why is this useful?
        \begin{itemize}
            \item 
        \end{itemize}
    \end{itemize}
    \item Provide more accurate estimates of the system. Why is this useful?
    \begin{itemize}
        \item Improve the accuracy of the state estimates.  Why is this useful?
        \begin{itemize}
            \item The more accurate our estimates, the more accurate we can control where we want to get to
        \end{itemize}
        \item Robust to sensor failures. Why is this useful?
    \end{itemize}
\end{itemize}


\begin{itemize}
    \item Manufacturing systems --- monitor tool wear \cite{shi2018using,pratama2019metacognitive,dou2020unsupervised,kuntouglu2021investigation,bleakie2013feature}, quality check \cite{lin2021metal,francis2019deep,shevchik2017acoustic}, predictive maintenance \cite{gu2017product,he2017integrated}, control the manufacture processing parameters \cite{},   --- \textbf{maximizing production, minimizing failure}
    \item Structural systems --- monitor for structural failure, input identifiability? ,... ---
    \item Biology --- classify and indicate the stages of yogurt fermentation reaction \cite{cimander2002sensor}, classify the type of honey \cite{ulloa2013determination},  detect mastitis in cows \cite{jensen2016bayesian} --- ???
    \item Gait cycles --- identify the phase of gait cycle \cite{meng2010emg,ziegler2018classification,zhao2019adaptive, horst2019explaining,alharthi2019deep}, predict ground reaction forces \cite{oh2013prediction}, control prothetics \cite{grimmer2016powered,guo2010study,hoover2012stair,au2005emg,huang2011continuous,zhang2019sensor}, detect gait anomalies  \cite{ajay2018pervasive, paragliola2018gait, bonetto2019seq2seq} like Parkinson's disease  --- \textbf{gait rehabilitation, health monitoring}
    \item Navigation systems, traffic systems --- navigation systems state estimation \cite{sasiadek2002sensor,hasan2009review,hansen2017nonlinear,shankar2019finite,rigatos2007extended,rigatos2010extended,yazdkhasti2018multi} --- \textbf{features can be estimated more accurately than with individual sensors and are robust to sensor failures}
\end{itemize}
}  

\textcolor{ForestGreen}{
\textbf{Sensor fusion in dynamical systems}
\begin{itemize}
    \item \cite{kelly2011visual,oskiper2012multi} - establishing observability of the sensors with known models and then fuse the sensors
    \item \cite{shen2019observability} - observability degree analysis for navigation to determine best sensor fusion method
    \item \cite{hu2018observable} - observability degree analysis for various sensor fusion architectures
    \item \cite{joukov2019estimation,madarash2004enhancing,nobahari2017application} - theoretical modeling for sensor fusion and observability analysis
    \item \cite{hol2006sensor,polychronopoulos2007sensor} - theoretical modeling later used for state estimation
    \item \cite{hegrenaes2007towards} - Sensor fusion for state estimation with application in control 
    \item \cite{sommeregger2017quality} - bioprocess - need for multivariate models to do better MPC of bioreactors
    \item \cite{teixeira2007hybrid} - Bioreactors - MPC using models with grey box identification
\end{itemize}
%  - 
}

\begin{comment}
\textcolor{blue}{
\textbf{Ideas of Paragraph 2: \textcolor{red}{ Do not like this formulation. It digresses too much and goes off topic. Redo!} Sensor fusion configurations using feature extraction and how they seep into different domains}
\begin{itemize}
    \item Types of configuration using feature extraction as the application
    \begin{itemize}
        \item Complementary- no real examples for this- use the temperature at different geographical locations as the example
        \item Competitive - INS position and orientation estimation from various sensor sources - handled by state estimation algorithms like Bayesian filtering and its variants -\textcolor{red}{another example is traffic systems - not using it for size constraints}
        \item Cooperative - multiple sensors are required to get a single feature and fails in the absence of even a single sensor - seen in gait cycles, \textcolor{red}{another example is manufacturing systems- ignored for size constraints}
    \end{itemize}
    \item An array of sensors can have a combination of these configurations. 
\end{itemize}
}
\end{comment}

\textcolor{blue}{
\textbf{Ideas of Paragraph 2: Enter Koopman operators- Explore KO as a sensor fusion approach}
\begin{itemize}
    \item \textbf{Why} Koopman operators for sensor fusion?
    \item \textbf{How} is KO used in sensor fusion?
    \item \textbf{What} is it that we want to do in KO for sensor fusion?
    \item \textbf{Notes:}
    \begin{itemize}
        \item We already talk about how sensor fusion is used to extract features and estimate states. If we start talking about the nonlinear state estimation, we might have to address. 
        \item Steer clear of offending anyone's work and try to say that you are proposing a new route
    \end{itemize}
\end{itemize}
}

\textcolor{blue}{
\textbf{Ideas of Paragraph 3: Model identification as a cooperative configuration problem and entry of Koopman}
\begin{itemize}
    \item Modeling with sensor fusion has typically been static (measurements to features) or dynamic (input-output models) which are typically nonlinear
    \item Koopman operator based sensor fusion
    \begin{itemize}
        \item traffic systems - \cite{avila2020data} analyze the forecast the dynamics
    \end{itemize}
    \item Koopman operators identify global linear representations of nonlinear models and have gained a lot of traction
\end{itemize}
}

\textcolor{ForestGreen}{\textbf{Koopman operator references?}
\begin{itemize}
    \item 
\end{itemize}
}



\textcolor{blue}{
\textbf{Ideas of Paragraph 4: What Koopman has and what Koopman needs?}
\begin{itemize}
    \item Koopman models do sensor fusion on the measured variables that constitute a full state of the system
    \item They identify the governing dynamics
    \item In this paper, we analyze how the addition of output measurements affect the Koopman identification problem. 
\end{itemize}
}

\textcolor{blue}{
\textbf{Ideas of Paragraph 5:}
\begin{itemize}
    \item 
\end{itemize}
}

\textcolor{blue}{
\textbf{Ideas of Paragraph 6:}
\begin{itemize}
    \item 
\end{itemize}
}
\newpage
.
\newpage

==> Abstract_and_Intoduction/old_intro_stuff.tex <==
Complementary configuration include scenarios like measuring temperatures at different geographical locations \cite{bachmann2011multi}. The measured variables do have any inter-dependency and can be directly concatenated to provide a more comprehensive picture. 

Feature extraction from data is a common problem in sensor fusion. When individual sensors can compute the same features independently, Bayesian filtering algorithm \cite{mitchell2007multi} which includes the well known Kalman filter and its variants implement competitive sensor fusion to estimate accurate feature estimates. 



Competitive configuration is seen in examples like the inertial navigation systems (INS) used in automotives and general aviation. Various sensors like the inertial mass unit (IMU) \cite{hasan2009review}, global navigation satellite system \cite{hansen2017nonlinear} and radio frequency beacons \cite{shankar2019finite} individually compute the same features of position and orientation of the INS. These independent computations of the same features can be integrated using the Bayesian filtering algorithm \cite{mitchell2007multi} which includes the well known Kalman filter and its variants \cite{sasiadek2002sensor,hasan2009review,hansen2017nonlinear,shankar2019finite,rigatos2007extended,rigatos2010extended,yazdkhasti2018multi}. The output of the algorithm yields more accurate estimates of the features than those provided by individual sensors and the estimation process is robust to sensor failures. 

Cooperative sensor fusion necessitates all sensor measurements be acquired to inform about the system and the lack of any measurement render incomplete or null information. Gait cycle monitoring is a good example where 

Cooperative and competitive sensor fusion problems discussed so far work under the assumption that a 


information from all sensors to extract the required features of the system.



These independent computations of the same features are integrated to get the most accurate feature estimates


Sensor fusion methods like Bayesian inference \cite{mitchell2007multi} which includes the well known Kalman filter and its integrate all the measurements

variants optimally estimate the state or feature from various measurements .

 In inertial navigation systems for general aviation, the same information of position and orientation are measured using various sensors like the inertial mass unit (IMU) \cite{hasan2009review}, global navigation satellite system \cite{hansen2017nonlinear} and radio frequency beacons \cite{shankar2019finite} independently. Using a combination of these measurements yields a competitive configuration and is typically handled by sequential Bayesian inference \cite{mitchell2007multi} which includes the well known Kalman filter and its variants to optimally estimate the state or feature from various measurements \cite{sasiadek2002sensor,hasan2009review,hansen2017nonlinear,shankar2019finite,rigatos2007extended,rigatos2010extended,yazdkhasti2018multi}. Competitive sensor fusion is typically used to make the system less sensitive to noise and robust to sensor failures. 

\textbf{Paragraph 3:}\\
Cooperative sensor fusion is the integration of the measured variables that have mutual information due to their inter-dependence. Capturing the underlying relationship between the measured variables and feature extraction are the core applications. Where models between the measurands and the features exist, the data is directly used for feature extraction. An example is in the gait cycle of humans and robots where various sensors like accelerometers, gyroscopes, magnetometers, EMG to extract gait cycle parameters like knee angle, swing time, swing angle, etc. \cite{tao2012gait}.

==> Abstract_and_Intoduction/old_stuff/Older_Abstracts.tex <==
We introduce the problem of learning deep neural network representations of the Koopman operator of a nonlinear dynamical system with output measurements that are sampled at a distinct timescale from the state.  We present an algorithm for solving the problem, output-constrained deep dynamic mode decomposition (OC-deepDMD) and show that the algorithm is effective at training neural network representations from data while simultaneously adapting the neural network embedding to predict an output function.  We analyze the properties of the output-constrained learning problem and show that increased output sampling resolution constrains the space of Koopman embeddings that can be realized, thereby reducing the underdeterminedness of the problem.  When the embedding space is bounded, we show convergence of output-constrained embeddings to a limiting set of output-constrained embeddings, which coincide with the embedding that predicts the entire output function as a continuously sampled function of time.  We illustrate this concepts with a numerical example from a simulated genetic circuit in synthetic biology.

\begin{comment}


\textcolor{red}{\textbf{The previous version}}

We introduce the problem of learning linear state space models of nonlinear dynamical systems with both state and output measurements. Koopman operator theory obtains a high dimensional linear state model from a low dimensional nonlinear system via a nonlinear transformation of the state which can be propagated linearly through time. We show that the addition of the output equation constrains the nonlinear transformation and that we can find a state-inclusive Koopman model with linear output under specific conditions. We present the output constrained deep dynamic mode decomposition (oc-deepDMD) algorithm to identify this model by training a neural network representation to identify the nonlinear transformation functions. We discuss two architectures - the direct oc-deepDMD jointly identifies both the state and output equations and the relatively sparse sequential oc-deepDMD identifies them separately. We analyze how the scaling of regressors for training the neural network affects the resulting Koopman model. We use numerical examples to illustrate the multistep predictive capability of the Koopman models identified by oc-deepDMD. We also use the example of an oscillator to show the limitations of the algorithm and how it can be overcome. 

\textcolor{red}{
\textbf{Comments I remember from the previous iteration:}
\begin{itemize}
    \item We aren't introducing a new problem. We are dealing with an existing one
    \item Many sentences are too verbose. Make sentences like how you make a conversation and not how you defend an argument.
    \item Too long sentences
    \item Use the why ? - how? and what? sequence
    \item We propose a new algorithm. Not present one
\end{itemize}
}

\textcolor{blue}{\textbf{The modified version}}
We consider the Koopman operator learning problem of nonlinear systems. \textcolor{violet}{The objective is to find a nonlinear transformation that lifts the states of the system to a high dimensional space where the system dynamics becomes linear in the lifted state space.} This is traditionally a grey box system identification problem with the prior assumption that all sensor measurements of the system constitute the state of the system and the lifting is identified on all the measurements. In some cases, the sensor measurements are classified as state and output measurement and joint sensor fusion Koopman model is identified. These cases have always assumed that the outputs lie in the span of the lifting functions making the output equation linear. This is a very strong assumption which is not always satisfied. Hence, this approach only seeks to identify a model that fits the state data well. In this paper, we remove that assumption and show how to identify Koopman operators that are constrained to make the output equation linear. Such models fit well to both the state and output data. We begin by showing that the output equation constrains the Koopman operator that can be identified. We also showed the existence of these output constrained Koopman operators with state inclusive lifting under the condition that both the state dynamics and output equation are analytic. To identify these models, we build on the existing deep dynamic mode decomposition (deepDMD) algorithm  proposed in \cite{yeung2019learning} which identifies the neural network representations of the lifting functions. We add the output constraint to the deepDMD objective function and propose the output constrained deepDMD (OC-deepDMD) problem. We put forward two algorithms that solves this problem - 1) the direct OC-deepDMD  jointly identifies the lifting functions by equally weighing the state and the output equations 2) the sequential OC-deepDMD which solves the state and output equation independently and then solves a third problem to fuse the two models. Among the two, the latter algorithm identifies relatively sparse models. We test these algorithms on three simulated examples in increasing order of complexity and show the successful identification of output constrained Koopman operators with limitations.


\textcolor{violet}{* I tried many different variants of explaining the Koopman operator learning problem and could use help here and I wanna ask is this even necessary- 
\begin{itemize}
    \item The objective is to find an injective nonlinear transformation of the states such that the nonlinear dynamics becomes linear in the high dimensional transformed state space.
    \item This constructs a high dimensional nonlinear transformation of the states such that the new states evolve linearly.
    \item The objective is to find high dimensional linear state space models of a given nonlinear system. This is done by lifting or embedding the states in a high dimensional plane using an injective nonlinear transformation such that the dynamics of the lifted states evolve linearly.
    \item The objective is to construct a high dimensional transformation of the state called the lifted states such that the nonlinear dynamics evolve linearly in these new states.
    \item The objective is to find a high dimensional transformation of the states called the lifted states such that the nonlinear dynamics evolve linearly in these newly constructed states. This enables us to use linear systems tools to study nonlinear dynamics. 
\end{itemize}}

\textcolor{red}{
\textbf{Shara's comments on this draft:}
\begin{itemize}
    \item The definitions should not form part of the abstract
    \item Keep the word count at 200
\end{itemize}
}
\end{comment}
\begin{comment}
We consider the Koopman operator learning problem of a nonlinear system where disparate sensors measure different facets of its dynamics. In specific, we ask how to construct Koopman operator representations from sensors that measure both the states and the outputs of the system? Traditionally, this is done by collecting all measured variables to constitute the concatenated state and lifting it to a high dimensional space where the dynamics are linear. The output equations capture the inter-dependency between the state and output variables and the validity of these models lie in the concatenated state space with these output equations as constraints. The drawback of this approach is that the validity space of the model is shrouded as the output equations are captured intrinsically in the model. In this paper, we pose the problem of learning Koopman operator models that explicitly capture these output equations. To preserve their linear structure, we focus on finding linear representations of the output equations. We show that by adding the output equation, we force a subset of the lifting functions to take the same structure as the output equations. We propose the output constrained deep dynamic mode decomposition (oc-deepDMD) algorithm to identify these output constrained Koopman operators (OC-KO). It uses neural network representations to approximate the lifting functions that simultaneously minimize the error in identifying linear representations of the state dynamics and output equation. We use three simulated examples in increasing order of complexity to show the success and limitations of the algorithm. These OC-KO models render linear models that are admissible throughout the state space, ensure that the outputs lie in the span of their lifting functions and successfully fuse the information from different types of sensor measurements. \textcolor{red}{Word count: 283}
\end{comment}
\begin{comment} We consider the Koopman operator learning problem of a nonlinear system where disparate sensors measure different facets of its dynamics. In specific, we ask how to construct useful Koopman operator representations fusing both state and output measurements? \textcolor{ForestGreen}{ We show that augmenting the state measurements with the outputs and using the traditional method of learning Koopman operators does not work. Such models capture the output equations intrinsically and as a consequence, they are neither useful for sensor fusion nor prediction on new initial conditions. Another approach is to assume that the outputs lie in the span of the observables. This assumption need not hold true. We show that the output equations constrain the lifting functions of the Koopman operator. Hence, we propose a new class of dynamic mode decomposition (DMD) problems where the Koopman operator learning problems is constrained on rendering linear representations of the output equations. In particular, we modify the deep DMD algorithm to identify these Koopman models. We use an example with an analytical solution to show that these models capture the governing dynamics of the system from data. Moreover, it also can separate out the eigenfunctions that contribute to the dynamics and the output. We use the example of an oscillator to bring out its limitation and discuss a potential method to bypass it.} The traditional approach is to collect all measured variables and form the concatenated state which is then lifted to a high dimensional space where the dynamics become linear. We show that such models capture the output equations intrinsically and \textcolor{red}{conceal their region of admissibility - \textbf{TOO COMPLEX}}. In this paper, we pose the problem of identifying sensor fusion models by learning Koopman operator models that explicitly capture linear representations of these output equations. We show that these output equations impose constraints on the lifting functions.  \textcolor{red}{We propose a new class of dynamic mode decomposition algorithms that embody the output constraints. We propose a new variant of the existing deep dynamic mode decomposition algorithm to embody the sensor fusion constraints and identify these models.} We use an example with an analytical solution to show that these models capture the governing dynamics of the system from data. Moreover, it also can separate out the eigenfunctions that contribute to the dynamics and the output. We use the example of an oscillator to bring out its limitation and discuss a potential method to bypass it. \textcolor{red}{Word count: 215 out of max 200}

We consider the Koopman operator learning problem of nonlinear systems where disparate sensors measure different facets of its dynamics. In specific, we ask how to construct useful Koopman operator representations by fusing the state and output measurements \textcolor{red}{for an autonomous nonlinear system with nonlinear outputs}?  We discuss why the traditional methodology of learning Koopman operators on all the measured variables is not a viable option in its current form. Such models capture the state to output relationships intrinsically and are rendered ineffective for sensor fusion and prediction purposes. We show that for Koopman operator models with linear output representations, the lifting functions are constrained by the nonlinear output equations of the system. We incorporate that information and pose a new class of dynamic mode decomposition (DMD) problems where such representations are identified by constraining the Koopman operator learning problem to yield linear representations of the output equations. In particular, we modify the deep DMD algorithm to identify these Koopman models. We use an example with an analytical solution to show that these models capture the governing dynamics of the system from data. Moreover, it also can separate out the eigenfunctions that contribute to the dynamics and the output. We use the example of an oscillator to bring out its limitation and discuss a potential method to bypass it. \textcolor{red}{Word count: 197 out of max 200}

We consider the Koopman operator learning problem of nonlinear systems where disparate sensors measure different facets of its dynamics. In specific, how do we construct useful Koopman operator representations that fuse state and output measurements?  The traditional method of learning Koopman operators on the concatenated measured variables is not a viable option in its current form. Such models capture the state to output relationships intrinsically and are rendered ineffective for state estimation and prediction purposes. To overcome this, we explore Koopman operator models with linear output representations. We show that their lifting functions are constrained by the nonlinear output equations of the system. We incorporate this information and pose a new class of dynamic mode decomposition (DMD) problems to learn Koopman operator models with a linear output equation constraint. To solve this, we propose the output constrained DMD algorithm and evaluate its performance using analytical and numerical examples. These algorithms identify useful sensor fusion Koopman operator models that can (1) utilize the outputs to inform the state (2) predict the evolution of states and outputs on new initial states and (3) pave the way to extend linear systems tools for observability analysis and observer design of nonlinear systems.
\end{comment}

==> Abstract_and_Intoduction/old_stuff/enoch_intro_old_one_with_RNASeqData.tex <==
Identifying models or governing equations to describe the dynamics of real-world physical systems can be challenging, especially when treating physical systems exhibiting nonlinear behavior.  System identification problems in this context can be categorized in terms of two objectives, first, identification and recovery of a faithful simulation of the system's dynamics in a way that {\it generalizes} to conditions or parametric points not observed in the training data, and second, identification and recovery of a faithful model that represents the underlying physical system's network structure and physical relationships between states or manifest variables.    A recurring theme of solving either objective in nonlinear system identification problems is that the data present is never sufficiently rich to constrain the discovery and selection of the nonlinear functions underlying the system's dynamics.   This makes these class of problems difficult to solve, without some additional insight or {\it a priori knowledge} of the system's structure. 

In this work, we consider a variant of the open-loop nonlinear system identification problem.  Recently we aimed to analyze time-series RNAseq data and reconcile it with fitness curves or growth kinetics, of bacterial cultures in microtiter plates.    The aim was to understand how whole-cell dynamics could be used to predict entire growth curves, which are a proxy of cellular fitness in a particular condition.   The problem is, at its core, a sensor fusion problem.  RNA sequencing provides a coarse-resolution glimpse into the average state of a culture of unsynchronized cells, reacting on a unified time-scale to some external stimulus, e.g. the sudden arrival of a new chemical analyte or metabolite or transfer into a novel media.    The growth kinetics, collected by a rapid scanning spectrophotometer, provide a bulk-culture read out of optical density, which provides a proportional readout of cellular density as a function of time.   RNA sequencing measurements are, by nature, expensive and labor intensive to collect, as they require the services of a deep sequencing instrument and a laborious RNA extraction, RNA library preparation, and sequencing library preparation process.   Spectrophotemeter measurements, or plate-reader measurements, are extremely cheap to collect in an automated fashion; it is possible to collect over a thousand timepoints during the course of a cell growth, i.e. fitness, assay.  Reconciling these measurements is thus a sensor fusion problem.  In this work, we treat the growth phenotype as an output function, a {\it particular} observable function, that is the desired projection of the system state represented by the RNA dynamics.    The former measurement is a low dimensional, scalar, and near-continuously sampled function, while the latter measurement is a high-dimensional and aggressively sampled function within a specified window of feasibility (when RNA extraction is feasible).   

Most generally we are considering a nonlinear time-invariant dynamic system with unknown governing equations, evolving on a defined notion of a system state $x \in \mathbb{R}^n$.  We suppose that the system can be measured sparsely at timepoints $x_1, ..., x_N$, while the output function can be measured precisely at those points as well $y_1 = h(x_1), ..., y_N = h(x_N)$ (and potentially in between state measurements).  We suppose that output measurements are available for many timepoints after the state measurements are collected, i.e. $y_{N+1} = h(x_{N+1}), ..., y_{N+k} = h(x_{N+k}).$    Our goal is to use these additional outputs to bootstrap the learning problem, to further constrain the space of nonlinearities, and to study the nature of the solutions to the system identification problem.  

To discover the class of nonlinearities that govern the system dynamics, we integrate the framework of deep learning and the theory of Koopman operator, to present a novel algorithm called output-constrained deep dynamic mode decomposition or (OC-deepDMD).   The algorithm presents a significant extension and revision of the {\it state-dependent} framework presented in deep dynamic mode decomposition \cite{yeung2019learning}, as it revises the flow of state and output variables to incorporate output-function constraints, propagated through multi-step Koopman operator predictions.   The algorithm  presents a novel perspective for the problem of output-constrained Koopman learning, as a complement to the problem of learning open-loop Koopman operators using deep neural networks, machine learning or dictionary approaches \cite{proctor2016dynamic,proctor2018generalizing,yeung2018koopmanGramian,williams2015data,williams2016extending,mezic2005spectral,lorsch2018,takeishi2017learning}.    As the output function of a physical system is the most manifest physical property of a dynamic system,  OC-deepDMD represents one of the first efforts into performing physics-informed Koopman operator deep learning \cite{stinis2019}.   The algorithm also represents a first attempt at using the Koopman operator method to address problems in sensor fusion, though notable efforts to construct Koopman operator representations in a wide range of physical systems (though not simultaneously) are abundant in the literature \cite{you2018deep,arbabi2019data,arbabi2017ergodic}.

==> Abstract_and_Intoduction/old_stuff/intro_3.tex <==

% Black box system identification is  obtaining a time-series model between the input and the output data without knowledge of the system. In addition, if we have some prior piece of information about the physics of the system, we can identify a better model by combining the physics-based information with the experimental data to identify a \textit{ grey-box model} as defined in \cite{bohlin2006practical}. In this paper, we explore systems where we have prior knowledge that some of the measured outputs are direct measurements of the full state of the system. Such models play an important role in scenarios like genotype to phenotype mapping in biological systems.  Identification of genes corresponding to a certain metabolic pathway \cite{atsumi2008metabolic,youngquist2013production,dal2011identification} or genes associated with traits like age at menarche, body mass index, breast cancer, etc. \cite{mancuso2017integrating,nacht1999combining,guo2020integrated,kellis2003sequencing} are some examples.  

% Consider the single cell bacterium \textit{Escherichia coli} in which a large network of genes interact to activate multiple metabolic pathways resulting in exhibiting multiple phenotypes as output at the same time. If we magnify on the gene interactions of a single phenotype, it can be seen that only a subset of genes is involved in expressing it - \textcolor{red}{\textbf{RESOLVE} find some papers on the phenotypes of E.coli}. Can we identify the subset of genes that express a single phenotype? In the state space framework, if we model the interaction of genes as a dynamical system with the collective gene expression as the state and the observed phenotype as the output, can we use observability analysis to shed light on the specific set of genes that contribute to the output. Moreover, with the state space model, can we query the dominant genes that affect that manipulate the phenotypic output? This system is highly nonlinear

% Consider the single celled microbe \textit{Escherichia coli}. There are various genes within the microbe that undergo transcription reactions to form mRNA(messenger ribonucleic acid) which in turn undergoes translation reactions to form proteins. These proteins exhibit a variety of functionalities like metabolism, cell growth, induce gene transcription, etc. thereby enabling the genes to interact with each other leading to a complex dynamical network. If we consider a phenotype of interest like cell population growth, can we map the evolution of the mRNAs and the corresponding proteins to that phenotype?  They use different methods of gene identification and can be formulated as a control problem. Not all genes are required to exhibit the phenotype of interest. Then the question naturally arises- can we identify a minimal list of genes that correspond to that phenotype? In control systems terminology, if me consider the mRNA and protein concentrations of various genes as the state that completely characterizes the system and the phenotype of interest as the output, then what we are essentially asking is to model the observable portion of the nonlinear system. In addition to offering a reduced model, what this yields is a significant cost reduction in the measurement process wherein instead of measuring all the mRNA concentrations using the more expensive RNA-sequencing experiments, we can use the cheaper real time quantitative polymerase chain reaction(rtqPCR) experiments to measure the minimalist genes of interest. 

==> Abstract_and_Intoduction/old_stuff/intro_5.tex <==
\begin{comment}


Identifying models or governing equations to describe the dynamics  of real-world  physical  systems  can  be  challenging, especially when they exhibit nonlinear behavior. The measured variables of the system dictate the type of model that can be identified. The simplest is the black box model where the measurements from all the sensors are treated as outputs of the system. This does not assume any prior knowledge of the measured variables. Some of the model structures developed that implement black box identification schemes are the Volterra series models \cite{schetzen1980volterra}, the Hammerstein models \cite{billings1979non}, the Weiner models \cite{guo2003identification, wang2008hammerstein} and the nonlinear autoregeressive exogenous input (NARX) model \cite{schoukens2009wiener, boussaada2018nonlinear}. A class of models called the nonlinear state space models map the input to the output via a set of hidden variables called the states \cite{nijmeijer1990nonlinear,khalil2014nonlinear}. Identification of these state space models from input-output data \cite{schon2011system,paduart2010identification} is also a black box identification technique.

Black box models do not encapsulate the physics of the system since we make no assumptions about the sensor data. On the other hand, white box models are purely physics based and their parameters are estimated from data. Grey box model structures include all that lie in between \cite{bohlin2006practical}. The Koopman operators \cite{mezic2005spectral} are a subclass of grey box models because they assume that the measurement variables collectively constitute the state of the system. Koopman operators lift the states of the nonlinear system by a suitable coordinate transform to an infinite dimensional lifted space such that the system dynamics evolve linearly in the lifted space. To identify infinite dimensional transformations is infeasible and hence we seek approximate finite representations. Dynamic mode decomposition (DMD) algorithm \cite{schmid2010dynamic} is commonly used to identify these finite representation Koopman operators. It does so by minimizing the error in two sub problems simultaneously. The first one is to identify a coordinate transformation that takes the states of the nonlinear system to the lifted states and back. The second one is to estimate a matrix transformation which propagates the lifted states linearly through time. 

\textcolor{red}{What more to write here?
\begin{itemize}
    \item DMD algorithms that are along the lines of just dealing with one set of measurements
    \item Do not try to give context on all the algo variants. Stick to the point.
\end{itemize}
}
Many variants of the DMD algorithm have been proposed \cite{arbabi2017ergodic,} to achieve the task in different ways. DMD algorithms have been adapted to accommodate more complex model structures that include inputs. 

\textcolor{red}{\textbf{Para: sensor fusion model problem intro- THE WHY HERE!}
\begin{itemize}
    \item Where do such cases rise?
\end{itemize}
}

The models discussed thus far deal with only one type of measurement. The black box models classify all the sensor data as outputs while the grey box models classify them as states. Naturally the question arises that what if we have data from disparate sensors such that some of the data represent the state of the system while others represent the output? Such examples arise in many fields like biology, aerospace, traffic systems... In biological systems, we can collect the data of the cell state by doing RNA sequencing experiment \cite{} which informs how many times have each gene been expressed called the genotype of the cells. We can collect phenotypic information of the cell as well by either observing the cell culture through microscope \cite{}, collecting fluorescence data \cite{} or the optical density at $600nm$ which informs the population of the cells \cite{}. How do we combine the genotypic information with the phenotypic information to create a useful model which allows us to study the underlying dynamical system?

Sensor fusion plays a pivotal role is such cases as it provides a framework for combining data from multiple sources

where the data from multiple sources is 


\textcolor{blue}{\textbf{Exercise for Shara: Use the power of three and bring out 3 key things that make up your work}
\begin{enumerate}
    \item Sensor fusion - only done in context of state estimation
    \item Sensor fusion model to study the underlying dynamics
    \item 
\end{enumerate}
}

\textcolor{blue}{\textbf{Sharad's paper}} In aerospace systems, sensor fusion of various measurements is required to estimate the position and orientation of the aircraft for accurate navigation. One such example is in \cite{shankar2019finite} where the measurements from the inertial mass unit and radio frequency measurement is fused 


The Koopman operators \cite{mezic2005spectral} which assume the measured output to be the state of the system are infinite dimensional linear state space models of finite dimensional nonlinear systems. Since they make a prior assumption that the measured output is the state of the system, they can be classified as grey-box models according to \cite{bohlin2006practical}. Finite representations of these Koopman operators are identified using the dynamic mode decomposition (DMD) algorithm \cite{schmid2010dynamic}.The Koopman operator framework has been developed for continuous time systems \cite{budivsic2012applied}, discrete time systems \cite{williams2015data,rowley2009spectral} and input-controlled systems \cite{proctor2016dynamic,williams2016extending}. Observability and controllability concepts have been established by constructing a Koopman gramian \cite{yeung2018koopmanGramian} and MPC using Koopman models is shown in \cite{korda2018linear}.

\end{comment}








==> Abstract_and_Intoduction/old_stuff/intro_6.tex <==
Modelling the dynamics  of real-world  physical  systems  can  be  challenging, especially when they exhibit nonlinear behavior. The required models of a system are determined by the application of study, but it is the set of measured variables that dictate which models can even be identified. The structure of these identifiable models are contingent on the data collected as well as prior knowledge about the system. In the absence of the latter, a typical strategy is to adopt the black box model structure which considers all measured variables as outputs of the system. The popular black box model structures for nonlinear system identification  include the Volterra series models \cite{schetzen1980volterra}, the Hammerstein models \cite{billings1979non}, the Weiner models \cite{guo2003identification, wang2008hammerstein} and the nonlinear autoregeressive exogenous input (NARX) model \cite{schoukens2009wiener, boussaada2018nonlinear}. The nonlinear state space models where the states of the model are treated as hidden variables \cite{schon2011system,paduart2010identification} are also black box models. They only capture the temporal relations in the data and not the physics of the process. On the other end, if complete knowledge of system is available, the white box models constitute the physics of the process with their parameters estimated from data. Grey box model structures constitute all that lie in between \cite{bohlin2006practical}. Koopman operator based models \cite{} are a category of grey box models because they assume that the set of all measured variables constitute the state of the system. 

Black box models and Koopman operator based models deal with only one type of measurement. The sensor data are entirely classified as outputs in the former and entirely as states in the latter. Naturally, the question arises- what if we have data that are a mix of both? Such scenarios are common in many fields like biology, aerospace, transportation systems... In biology, diverse sensor data which give different information about the biological cell systems are available. While data like RNA sequencing measurements \cite{} and proteomics measurements \cite{} measure the activity within the cell, others data like microscopic images \cite{} and the optical density at $600nm$ \cite{} observe characteristics of the cell from the outside. Inertial navigation systems for cars and general aviation use an inertial measurement unit \cite{hasan2009review} to measure the position and orientation internally. Global navigation satellite system \cite{hansen2017nonlinear} and radio frequency beacon measurements \cite{shankar2019finite} are some of the external measurements that can be used to estimate the same information. Transportation management centers aim to monitor and control traffic using measurements from route trackers, Bluetooth, loop detectors...\cite{bachmann2011multi}. In all the scenarios, how do we combine the various sensor information to study the system dynamics?

The coalescence of different types of measurements to render information in some sense better than that would be possible when only individual sensor data were used is the area of sensor fusion \cite{bachmann2011multi}. In the case of the navigation systems and the transportation systems mentioned, the relation between the measured variables and the states of the system is modeled using the physics of the system and the main task is to fuse the various estimates of the states. This is done using the Kalman filter architectures \cite{bachmann2011multi,hasan2009review,hansen2017nonlinear} and maximum likelihood estimates \cite{shankar2019finite}. This luxury is not extended to the complex biological systems. While some organisms like \textit{Escherichia coli} \cite{} have a well mapped dynamics, novel organisms like \textit{Vibrio natriegens} \cite{} and \textit{Pseudomonas fluorescens} \cite{} are still a mystery box. Hence there is a need to study develop a method to fuse the data from various sensors to identify models that inform the dynamics of the system. In this paper, we focus on developing models of systems that fuse the state and output measurement to give a complete picture of the underlying dynamics.

To identify sensor fusion models that combine both state and output measurements to inform the dynamics of the system, we consider the grey box model structures. With the state and output variables clearly defined, the state space models can be used as we have information about the state. The nonlinear state model captures how the state changes as a function of time and the nonlinear output model captures independently how the state maps to the outputs. But the model structure is nonlinear. Koopman operators are of specific interest because of their ability to construct global linear models of nonlinear systems and inform about the prominent dynamic modes in the system. Koopman operators identify a nonlinear transformation that lifts the states of the system to a high dimensional space where the system dynamics becomes linear in that lifted state space. Finite representations of these Koopman operators are identified using the dynamic mode decomposition (DMD) algorithm \cite{schmid2010dynamic}. When we have both state and output measurements, one of the approaches in Koopman operator theory is to consider all the variables to be the state as done in \cite{korda2018linear} to consider linear predictor models for model predictive control. Another method is to assume that the outputs lie in the span of the transformed states \cite{yeung2018koopmanGramian,surana2016koopman,hasnain2019optimalReporterPlacement}. This is a very strong assumption which is not always satisfied. In this paper, we remove this assumption and establish the theory and algorithms to identify Koopman operators that make both the state dynamics and the output equation linear. Since these Koopman operators are identified by imposing the output equation to be linear, these are called output constrained Koopman operators (OC-KO). We begin by showing that the outputs constrain the lifting functions of the OC-KO. We also show that we can find state-inclusive non linear transformation for the OC-KO. 

To identify the OC-KO models, we build on top of the deepDMD algorithm from \cite{yeung2019learning}. We choose this algorithm as it does not require us to specify the lifting functions. It harnesses the power of neural network representations to identify the lifting functions while simultaneously solving for the linear transformation matrix of the lifted states. We modify the objective function by adding the linear output constraint to facilitate the identification of OC-KO. We propose two methods to solve this problem - 1) direct OC-deepDMD algorithm directly identifies the lifting functions that jointly make both the state and output equations linear 2) sequential OC-deepDMD algorithm solves two problems to identify the lifting functions for the state and output separately and then a third problem to identify the lifting functions that fuses them both. We evaluate the algorithms on three simulation examples of nonlinear systems with nonlinear output in increasing orders of complexity - 1) system with a theoretical finite Koopman operator representation, 2) system without a finite representation but with one equilibrium point and 3) system with a limit cycle. We compare the performances of the two algorithms with either the theoretical solution or the grey box nonlinear state space representation identified by neural networks to bring out the advantages and the limitations of the algorithms.

\textcolor{red}{Like it from a previous writing to talk about the type of sensor configurations- competitive, complementary or collective}
What if the sensors provide measurements that contain both states and outputs? Sensor fusion is the domain that combines the information from multiple sensors to provide better information about the system than that would be possible with individual sensors \cite{bachmann2011multi}. Based on the type of information provided by the sensors, sensor fusion has three different sensor configurations. In the inertial navigation systems for cars and general aviation, the inertial mass unit (IMU) \cite{hasan2009review}, global navigation satellite system \cite{hansen2017nonlinear} and radio frequency beacon measurements \cite{shankar2019finite} have a \textit{competitive} configuration as all of them estimate the same information of position and orientation. The accelerometers and gyroscopes in the IMUs provide measurements of distinct pieces of information like the linear acceleration or the rotation rate in three orthogonal directions. These sensors function in a \textit{complementary} configuration to give a complete picture of the position and orientation. When the IMU is used to calculate parameters like . In the above examples, the type of configuration could be established because the relationship between the variables of interest and the measured variables is established. But in fields like biology, disparate instrumentation techniques provide different pieces of information about the system. While transcriptomics \cite{wang2009rna} and proteomics \cite{aebersold2003mass} data study the gene and protein activity respectively within the cells, instruments like microscopes\cite{lefman2004three}, plate readers\cite{meyers2018direct} and flow cytometers \cite{gant1993application} study morphological traits like fluorescence and population growth. Biology has evolved by gaining significant insights by considering all these data independently. A combination of the various instrumentation techniques and the fusion of their data could lead to holistic picture and far more insights. But to do so, we need to develop model structures that can work hand in hand with sensor fusion. In this paper, we attempt to leverage the power of Koopman operators to identify sensor fusion models and study the effects of sensor fusion on identifying the Koopman operator representations. 

Many numerical methods for identifying Koopman operators from data have been developed in the last two decades \cite{askham2018variable,kaneko2019convolutional,azencot2019consistent,manohar2019optimized,schmid2010dynamic,sinha2019computation,yeung2019learning,hasnain2019data}.  The most common approach is to use dynamic mode decomposition (DMD), which models nonlinear dynamics via an approximate local linear expansion \cite{schmid2010dynamic}.  In \cite{williams2015data} an extended dictionary of basis functions with universal function approximation properties is used to discover an approximation of the lifting map or observables. These techniques suffer from combinatorial explosion, which generally has prohibited analysis of high-dimensional nonlinear systems \cite{Johnson2018class}. The most recent developments in the field of DMD integrate established advances in deep learning with DMD \cite{yeung2019learning,otto2019linearly,takeishi2017learning,li2017extended} where the deep neural networks have the capacity to approximate exponentially many distinct observable functions. Recent work has shown deep Koopman learning algorithms can be extended to synthesize controllers for systems subject to uncertainty \cite{you2018deep}, suggesting that deep Koopman learning can be used broadly for robust controller synthesis.

Koopman operators identify a nonlinear transformation that lifts the states of the system to a high dimensional (potentially infinite) space where the system dynamics become linear. Finite representations of these models are identified in practice. The most common approach to identify Koopman operators is using the dynamic mode decomposition (DMD) algorithm \cite{schmid2010dynamic} which constructs accurate models for linear systems and local linearized models for nonlinear systems. Many variants of the DMD algorithm have been proposed \cite{askham2018variable,kaneko2019convolutional,azencot2019consistent,manohar2019optimized,sinha2019computation,yeung2019learning,hasnain2019data} to identify Koopman operators of nonlinear system which are valid for bigger regions of the phase space. Koopman operators have been extended to include input-control \cite{proctor2016dynamic,williams2016extending,mezic2015applications,korda2018linear}. Very limited research has been done in extending Koopman operators to include outputs. 

==> Abstract_and_Intoduction/old_stuff/shara_intro_in_context_of_synthetic_biology.tex <==
Redesigning an organism to equip it with various constructive functionalities is the field of synthetic biology. Microorganisms are tailored for various applications like biosensing of changing conditions and harmful substances in the environment, bioremediation of soil, air and water and modulating metabolic pathways to yield useful products. Enzyme based reactions to implement Boolean logic circuits have been discussed in \cite{voigt2006genetic} and using differential enzyme expression in pathological conditions as the sensing mechanism is discussed in \cite{windmiller2010boolean},\cite{halamek2010multiplexing} and \cite{manesh2009enzyme} and an extensive review of literature is provided in  \cite{teravest2011bacteria}. In \cite{atsumi2008metabolic}, the metabolic pathway of 1-butanol from biomass is identified in other species of bacteria and the pathway has been successfully implemented in \textit{E.coli} and similar strategies for other products have been adopted in \cite{yim2011metabolic},\cite{shen2008metabolic} and \cite{lee2007systems}. Though promising results have been obtained, the efficiency of the experimental pipeline can be increased by taking the dynamical and control systems approach. 

Dynamical systems analysis offers a useful platform to formulate the above problems in a mathematical framework to model the dynamics as a function of the state to answer questions of controllability and observability of the states {\color{red} which could represent the gene expression, enzyme concentration, cell population and so on EY: too many dependent clauses in this sentence ——— run on sentence}. By addressing the observability problems {\color{red} vague reference/language}, we can identify the optimal genes to monitor based on the required functionality {\color{red} indirect referencing and tense, use direct and active tense} and by solving the controllability problem, we can identify the optimal genes whose expression can be controlled by actuators like CRISPR and its variants {\color{red} too many dependent clauses}. A good example of this methodology is illustrated in \cite{hasnain2019optimalReporterPlacement} where the Koopman observability gramian of a nonlinear system developed in \cite{yeung2018koopmanGramian} is maximized to locate the optimal reporter placement for maximizing the output of a genetic network.

High dimensional, nonlinear and time varying nature of the biological systems due to the various genomic interactions, the myriad metabolic pathways and the non-selective mutations pose a challenge for an adequate model identification {\color{red} not a sentence, revise!}. Several frameworks for nonlinear system identification from the input-output data have been developed. Some popular ones are the Volterra and Weiner series \cite{schetzen1980volterra} model where the relationship between the input and the output is expressed in terms of kernel functions based on the Taylor series expansion and the nonlinear autoregressive models with exogenous inputs (NARX) a finite amount of past inputs and outputs are related to the current output via a nonlinear function with the nonlinearity being polynomial\cite{lind2008regressor}, neural networks\cite{diaconescu2008use}, wavelets\cite{billings2005new} and so on. Though these models work well in prediction, their structure is not suited for controllability and observability analysis. Hence, we turn towards the Koopman operator \cite{mezic2005spectral} which is a mathematical construct for a nonlinear system evolving in linear basis to be transformed into a linear system evolving in a nonlinear basis. The Koopman operator framework has been developed for continuous \cite{budivsic2012applied} and discrete time systems \cite{williams2015data,rowley2009spectral}, for open-loop \cite{williams2015data} and input-controlled \cite{proctor2016dynamic,williams2016extending} dynamic systems.  Koopman operators generically can be divided into two categories, those with discrete (countable) spectra \cite{williams2015data} and those with (uncountable) spectra \cite{mezic2005spectral}.

Koopman operators are identified using the numerical algorithm- Dynamic Mode Decomposition(DMD) which models the nonlinear dynamics via an approximate linear expansion\cite{schmid2010dynamic}. Many variants of this algorithm have been developed over the years for various purposes - the extended DMD \cite{williams2015data} which constructs an extended list of basis functions, the Hankel DMD\cite{arbabi2017ergodic} which uses a finite length of the time series data as the state, the Causal Jump DMD \cite{balakrishnanprediction} which is a fusion of the two and so on. Deep DMD\cite{yeung2019learning} is the most recent advent in the class of DMD algorithms since it deploys a neural network to identify the nonlinear basis functions on which the linear model can be built. 

==> Abstract_and_Intoduction/sensor_fusion_definition.tex <==
Sensor fusion encompasses the tools, techniques and tools which are used for combining sensor data, or data derived from sensory data, into a common representational format.

==> Abstract_and_Intoduction/wow_opening_lines.tex <==
Sensors are proliferating across countless dynamical systems measuring different features of the system. 

What I want to say?
Sensor tech has evolved in many many applications to gain knowled


Knowledge about the unknown is made possible by using sensors and s

In the past two decades, the rapid rise in the capabilities of
sensor systems involving analytical computing technologies
has allowed the extraction of richer information from an
increasing number of sensing modalities.

a huge amount of heterogeneous data are collected by a variety of sensors. The
increasing accessibility and diversity of the data resources provide new opportunities for structural health monitoring,
while the aggregation of information obtained from multiple sensors to make robust decisions remains a challenging
problem

automated target recognition, environmental monitoring, robotics, medical applications, quality control
of manufacturing process, and condition monitoring of
complex machinery.




==> example_systems/Genotype-Phenotype_map_using_RNAseq___OD600_data.tex <==
\newpage
\section{Genotype - Phenotype Map}

\textcolor{blue}{\textbf{Things to do:}
\begin{itemize}
    \item Include the sampling theorem along with the scaling theorem and group them under the title of "Practical considerations"
    \item Reference it in the abstract
    \item Reference it in the intro
    \item Write about the experimental data procured
    \item Make sure reference to any Theorem, Section, Corollary, ... is always capitalized
\end{itemize}}

\textbf{A lil bit about the data acquired: } We use the growth curve experimental data in \cite{balakrishnan2020prediction} to determine that the soil microbe \textit{Pseudomonas putida} KT2440 exhibits maximal growth in R2A media with $3.51 g/L$ casein hydrolysate and $0.146 g/L$ glucose. For this maximal growth condition, we acquire two datasets: 
\begin{enumerate}
    \item the RNA sequencing (RNAseq) data of the genome with a sampling time of $1 hr$ to represent the state of the system
    \item the optical density at 600nm (OD600) using a plate reader with a sampling time of $3 mins$ to represent the output, a function of the state. 
\end{enumerate}

Using Theorem \textcolor{red}{\textbf{?}}, we concatenate the output data across time to enable the usage of OC-deepDMD algorithm. 

\textbf{Models to be fit}
\begin{itemize}
    \item 
\end{itemize}

==> example_systems/Unused_tables.tex <==
% \begin{table}[t]
% \begin{center}
% \centering
% \caption{The identified Koopman operator representation models for Example \ref{example theoretical closure} and their corresponding best model performance}
% \begin{tabular}{cccccc}
% \toprule
% Model & Data& Algorithm & \# Lifting & $r^2_{test}(x)$ & $r^2_{test}(y)$\\   
%  No &  &  & functions & (n-step) &  \\
% \midrule
%   1 & x & deepDMD & 4 & 1 & -\\
%   2 & x,y & dir oc-deepDMD & 4 & 0.93& -0.14\\
%   3 & x,y & dir oc-deepDMD & 6 & 1 & 1\\
%   4 & x,y & seq oc-deepDMD & 6 & 1 & 1\\
%   \bottomrule
% \end{tabular}\label{Table: Eg1 models and their performance}
% \end{center}
% \vspace*{-3mm}
% \end{table}

% \begin{figure}[t]
% \centering
%   \includegraphics[width=\textwidth/2,keepaspectratio]{images/MEMS_phase_portrait.png}
%   \caption{Phase portrait of the identified models capturing the dynamics of the  MEMS actuator }\label{fig: eg_MEMS_phase_portrait}
%   \vspace*{-5mm}
% \end{figure}
% Though the n-step predictive capability of the oc-deepDMD models are worse than the neural network model, it can be seen in Figure \ref{fig: eg_MEMS_phase_portrait} that the phase portrait is almost accurately captured with a high correlation. 

% \begin{table}[t]
% \begin{center}
% \centering
% \caption{Performance metrics of the optimal Koopman operator representation models identified for Example \ref{example Nonlinear MEMS resonator with differential capacitor}}
% \begin{tabular}{ccccc}
% \toprule
% Model & Algorithm & $r^2_{test}(x)$ & $r^2_{test}(x)$ & $r^2_{test}(y)$ \\
% No & used & 1-step & n-step & \\
% \midrule
% 1 & neural network  & 0.9999 & 0.9984 & 0.9997\\
% 2 & dir oc-deepDMD  & 0.9998 & 0.84 & 0.995\\
% 3 & seq oc-deepDMD  & 0.9991 & 0.883 & 0.999\\
%   \bottomrule
% \end{tabular}\label{Table: MEMS models and their performance}
% \end{center}
% \vspace*{-3mm}
% \end{table}

% \begin{table}[t]
% \begin{center}
% \centering
% \caption{Performance metrics of the optimal Koopman operator representation models identified for Example \ref{example activator repressor 2 state}}
% \begin{tabular}{cccccc}
% \toprule
% Model & Algorithm & $n_d$ & $r^2_{test}(x)$ & $r^2_{test}(x)$ & $r^2_{test}(y)$ \\
% No & used & & 1-step & n-step & \\
% \midrule
% 1 & neural network & 1 & 0.9999 & 0.8539 & 0.9968\\
% 2 & dir oc-deepDMD & 1 & 0.9994 & 0.5301 & 0.9827\\
% 3 & seq oc-deepDMD & 1 & 1 & 0.3488 & 0.9981\\
% % 4 & dir oc-deepDMD & 4 & 0.9994 & 0.5301 & 0.9827\\
% % 5 & dir oc-deepDMD & 5 & 0.9994 & 0.5301 & 0.9827\\
% 4 & dir oc-deepDMD & 6 & 0.9947 & 0.9116 & 0.8791\\
% % 7 & dir oc-deepDMD & 7 & 0.9994 & 0.5301 & 0.9827\\
% \bottomrule
% \end{tabular}\label{Table: Activator-Repressor models and their performance}
% \end{center}
% \vspace*{-3mm}
% \end{table}


==> example_systems/system_combinatorial_promoter.tex <==
\begin{example}\label{example combinatorial promoter}
Combinatorial Promoter System
\end{example}  
The combinatorial promoter system entails the dynamics of transcription of a gene in the presence of both activators and repressors as transcription factors with each transcription factor induced by an inducer and the promoter of the lac system is a good example \cite{del2015biomolecular}. The CAP activator which is positively induced by cAMP and LacI repressor which is negatively induced by lactose control a single promoter of the lac system thereby controlling the expression of genes for metabolizing lactose. Moreover, the cAMP inducer is expressed only when there are low glucose levels and hence, only when both glucose and lactose are absent can the proteins for metabolizing lactose even be expressed. We model the dynamics using the transcription equations coupled with the dynamics of the two inducers, activator and repressor given by:
\begin{align*}
    \dot{x}_1 =& -k_{1f}u_1x_1 + k_{1r}x_5\\
    \dot{x}_2 =& -k_{2f}u_2x_2 +k_{2r}x_6 - k_{4f}x_2x_3\\
    &+ k_{4r}x_8 - k_{5f}x_2x_7 + k_{5r}x_4\\
    \dot{x}_3 =& -k_{3f}x_3x_5 + k_{3r}x_7 - k_{4f}x_2x_3 + k_{4r}x_8\\
    \dot{x}_4 =&-k_{7f}x_4x_7 +k_{7r}x_{10} + k_{8f}x_{10}\\
    \dot{x}_5 =&k_{1f}u_1x_1 - k_{1r}x_5 -k_{3f}x_3x_5 \\
    &+ k_{3r}x_7 -k_{6f}x_5x_8 + k_{6r}x_4\\
    \dot{x}_6 =& k_{2f}u_2x_2 -k_{2r}x_6\\
    \dot{x}_7 =&k_{3f}x_3x_5 - k_{3r}x_7 - k_{5f}x_2x_7 + k_{5r}x_4\\ 
    & -k_{7f}x_4x_7 +k_{7r}x_{10} + k_{8f}x_{10}\\
    \dot{x}_8 =& k_{4f}x_2x_3 - k_{4r}x_8 -k_{6f}x_5x_8 + k_{6r}x_4\\
    \dot{x}_9 =&k_{5f}x_2x_7 - k_{5r}x_4 + k_{6f}x_5x_8 - k_{6r}x_4\\
    \dot{x}_{10} =& k_{7f}x_4x_7 -k_{7r}x_{10} - k_{8f}x_{10}\\
    \dot{x}_{11} =& k_{8f}x_{10} - \delta x_{11}\\
    y(t) =& \frac{1}{1+(K_a/x_{11})^{0.5}}
\end{align*}
where $u_1$ is the concentration of inducer(Ind1) for activator(Act) whose conc. is $x_1$, $u_2$ is the conc. of inducer for repressor(Ind2) whose conc. is $x_2$, $x_3$ is the DNA-promoter(DNAp) conc., $x_4$ is the RNA-polymerase(RNAP) conc., $x_5,x_6,x_7,x_8,x_9 \text{ and } x_{10}$ are the conc. of the reaction intermediates Act:Ind1, Rep:Ind2, DNAp:Act:Ind1, DNAp:Rep, DNAp:Act:Ind1:Rep and RNAP:DNAp:Act:Ind1 respectively. $x_11$ is the conc. of the mRNA formed, $k_{if}$ and $k_{ir}$ are the forward and reverse reaction coefficients of the $i^{th}$ reaction and $\delta$ is the degradation rate of the mRNA. \textcolor{red}{ We model the output as if the mRNA is fluorescent} and the fluorescent output equation is given by
\begin{equation*}
    y(t) = \frac{1}{1+(K_a/x_{11})^{0.5}}.
\end{equation*}
Since $u_1$ and $u_2$ are the inputs to the system and the purpose of the paper is to deal mainly with state-output equations, we take the inputs to be a constant value of $5.0$ and $2.0$ respectively. 

==> example_systems/system_glycolytic_oscillator.tex <==
\begin{example}\label{example glycolytic oscillator}
    Glycolytic Oscillator
\end{example}

The yeast glycolytic oscillator model is a common test case in biochemical systems. We consider the system in \cite{daniels2015efficient} along with an output equation which is formed by the fluorescence of the protein $x_7$ given by
\begin{align*}
    \dot{x}_1 =& J_0 - \frac{k_1x_1x_6}{1+(x_6/K_1)^q}\\
    \dot{x}_2 =& 2\frac{k_1x_1x_6}{1+(x_6/K_1)^q} - k_2S_2(N-S_5) - k_6x_2x_5\\
    \dot{x}_3 =& k_2x_2(N-x_5) - k_3x_3(A-x_6)\\
    \dot{x}_4 =& k_3x_3(A-x_6) - k_4x_4x_5 - \kappa(x_4-x_7) \\
    \dot{x}_5 =& k_2x_2(N-x_5) - k_4x_4x_5 - k_6x_2x_5 \\
    \dot{x}_6 =& -2\frac{k_1x_1x_6}{1+(x_6/K_1)^q} + 2k_3x_3(A-x_6) -k_5x_6\\
    \dot{x}_7 =&\mu\kappa(x_4-x_7) -kx_7\\
    y(t) =& \frac{1}{1+(K_a/x_{7})^{0.5}}
\end{align*}

The parameters used for the simulation are $J_0 = 2.5, N=1,A=4, k_1 = 100,k_2 = 6, k_3 = 16, k_4 = 100, k_5 = 1.28, k_6 = 12, k_7 = 1.8, K_1 = 0.52, \kappa = 13, \mu = 0.1, q=4, K_a = 1$ and this yields an oscillatory behaviour. The initial conditions are $x_1 \sim {\cal U}(0.8,1.6),x_2 \sim {\cal U}(1.08,2.16),x_3 \sim {\cal U}(0.1,0.2),x_4 \sim {\cal U}(0.175,0.35),x_5 \sim {\cal U}(0.15,0.3),x_6 \sim {\cal U}(1.335,2.67) \text{ and }x_7 \sim {\cal U}(0.05,0.1)$ where ${\cal U}$ indicates a uniform distribution. We simulate 300 curves with a sampling time of $0.5 s$ and a simulation time of $5s$ for each curve. For any system above two states, it is difficult to construct phase portrait and eigenfunctions as we require numerous projections and hence, are not considered for this example. 

\begin{figure*}
  \includegraphics[width=\textwidth]{images/eg4_GlycolyticOscillator.png}
    \caption{(a) 1-step and n-step predictions of sequential oc-deepDMD model on a test data-set (b) n- step predictive accuracy comparison across the models obtained by direct oc-deepDMD(Dir ocdDMD), sequential oc -deepDMD (Seq ocdDMD) and Hammerstein neural network (Hamm-nn) (c) Temporal evolution of the eigenfunctions}\label{fig: eg_GlycolyticOscillator}
\end{figure*}

==> sections/99_not_included_files.tex <==
% \begin{comment}


% \section{Mathematical Analysis of Input-Constrained Koopman Operators}\label{sec: Mathematical Results}


% % output observables are projections of Koopman eigenfunctions, every observable can give a pseudo-inverse based approximation of a Koopman eigenfunction, given Wh 
% % an output constrained learning problem requires that output is in the span of Wh and simultaneously, f(x) = K_{U} \psi_x(x)




% % \begin{theorem} \label{thm: parsimony of Koopman input}


% \subsection{Modeling additional actuators}
%  To tackle the actuator placement problem, we add more inputs $w_i$ to the nonlinear system (\ref{eq: NL system}) multiplied by the corresponding Boolean variables $k_{w_i} \in \{0,1\}$ to dictate the admissibility of the various actuators and this can be combined together to form the super system
% \begin{equation}
%     \begin{split}
%         \dot{x} &= \Tilde{f}(x,u,w)\\
%         w &=[k_{w_1}w_1 \quad k_{w_2}w_2 \quad \cdots \quad k_{w_q}w_q]
%         \label{eq: super NL system} 
%     \end{split}
% \end{equation}
% where $\Tilde{f}:\mathbb{R}^{n}\times \mathbb{R}^{m}\times \mathbb{R}^{q}\rightarrow \mathbb{R}^n$ is an analytic function  $x \in \mathbb{R}^n$, $ u \in \mathbb{R}^m$ and $ w \in \mathbb{R}^q$. If $w=[0\quad 0 \cdots0]^T$, then $F(x,u,0)=f(x,u)$ and recover the original nonlinear system (\ref{eq: NL system}). We can decompose this system as
% \begin{equation}
%     \dot{x} = f(x,u)+ g(x,u,w) 
% \end{equation}
% \begin{assumption}\label{assump: NL super system independent inputs}
%     The new actuator inputs $w_i$ affect the dynamics of the nonlinear super system (\ref{eq: super NL system}) independent of each other.
% \end{assumption}
% Using assumption \ref{assump: NL super system independent inputs}, we can decompose $g(x,u,w)$  into individual terms with each term containing the additional dynamics contributed by a single input $w_i$ and since $k_{w_i}$ is an dynamics admissibility term, it can be taken out of the nonlinear equation as
% \begin{equation}
%         g(x,u,w) = \sum_{l=1}^q g^{(l)}(x,u,k_{w_l}w_l) = \sum_{l=1}^q k_{w_l}g^{(l)}(x,u,w_l)\nonumber \\
% \end{equation}
% If we construct the same list of observables as in (\ref{eq: Koop_input complete matrix}), then for each observable ($\psi^{(1)}_i$ used as a shorthand for $\psi^{(1)}_i(x)$)
% \begin{equation}
%     \begin{split}
%         \dot{\psi}^{(1)}_i &= \nabla_x^T\psi^{(1)}_i f(x,u) +\sum_{l=1}^q k_{w_l}\nabla_x^T\psi^{(1)}_i g^{(l)}(x,u,w_l)\nonumber \\
%     \end{split}
% \end{equation}
% where $\nabla_x^T=[\frac{\partial}{\partial x_1} \quad \frac{\partial}{\partial x_2}\cdots \frac{\partial}{\partial x_n}]$. Concatenating all of the observable dynamics yield:
% \begin{equation}
%      \dot{\psi}^{(1)}=
%     \nabla_x^T\psi^{(1)}\Big{(}f(x,u) + \Tilde{G}\Tilde{k}_w
%     \Big{)} 
% \end{equation}
% \begin{equation}
%     \psi^{(1)} = \begin{bmatrix}
%         \psi^{(1)}_1\\
%         \psi^{(1)}_2\\
%         \vdots\\
%         \psi^{(1)}_N
%     \end{bmatrix}
%     \Tilde{G} = \scalebox{0.9}{\begin{bmatrix}
%         g^{(1)} & 0 & \cdots & 0\\
%         0 & g^{(2)}  & \cdots & 0\\
%         \vdots & \vdots & \ddots & \vdots\\
%         0 & 0 & \cdots & g^{(n)}
%     \end{bmatrix}}
%     \Tilde{k}_w = \begin{bmatrix}
%         k_{w_1}\\
%         k_{w_2}\\
%         \vdots\\
%         k_{w_n}
%     \end{bmatrix}\nonumber
% \end{equation}

% Substituting relevant terms based on equations (\ref{eq: Koop_input complete matrix}) and (\ref{eq: NLsys differentiated}) and concatenating all the states yield
% \begin{equation}
%     \begin{split}
%         \dot{\psi}^{(1)}(x) &= \mathcal{K}_{x} \psi^{(1)}(x) + \mathcal{K}_{xu} \psi^{(2)}(x,u)\\
%         &+ \mathcal{K}_{u} \psi^{(3)}(u) + \nabla_x^T\psi^{(1)}\Tilde{G}(x,u,w)\Tilde{k}_w\\
%     \end{split}\label{eq: NL multi input}
% \end{equation}
% This is the form of the equation to be used if the dynamics of the actuators are known. If the dynamics are to be identified, we need to look at the Koopman representation of the additional term. 

% \subsection{\textbf{\textcolor{red}{PROBABLY REMOVING THIS SUBSECTION}} Optimal sparse actuator placement}
% Given the Koopman model and the dynamics of the various actuators under consideration, we now turn our attention to identifying the optimal actuators for output reference tracking. We append the actuator dynamics to the Koopman 
% \begin{equation}
%     \begin{split}
%         \psi^{(1)}(x_{k+1})= &\mathcal{K}_{x} \psi^{(1)}(x_k)+\mathcal{K}_{xu}\psi^{(2)}(x_k,u_k)\\
%          &+\mathcal{K}_{u} \psi^{(3)}(u_k) +\mathcal{W}_k\Tilde{k}_w\nonumber \\
%         y_k =& \mathcal{W}_{h}\psi^{(1)}(x_k)
%     \end{split}
% \end{equation}
% where $ \mathcal{W}_k \in \mathbb{R}^N$ is a collection of dynamics of all the additional inputs in the nonlinear form (\ref{eq: NL multi input}) or the Koopman form (\ref{eq: Koop multi input})  such that
% \begin{equation}
%     \mathcal{W}_k = [
%         \Tilde{\mathcal{K}}_{xuw_1} \Tilde{\psi}^{(1)}  \quad \Tilde{\mathcal{K}}_{xuw_2} \Tilde{\psi}^{(2)}   \cdots \Tilde{\mathcal{K}}_{xuw_n} \Tilde{\psi}^{(n)}]\nonumber
% \end{equation}
% where $ \Tilde{\psi}^{(i)} = \Tilde{\psi}^{(i)}(x,u,w_i) $ is the dictionary of Koopman observables pertaining to the input $w_i$. Now, given the input sequence $u_k$ and a target output $y^t_k$, we now pose the integer programming optimization problem that chooses the $N_{actuators}$ best optimal actuators that can approximate the target dynamics
% \begin{equation}
%     \begin{split}
%         \min_{\Tilde{k}_w} &\sum_k||y_k^t - \mathcal{W}_h\psi_1(x_k)|| \\
%         \text{subject to} \quad 
%         \psi_1(x_{k+1})&= \mathcal{K}_{x} \psi_1(x_k)+\mathcal{K}_{xu}\psi_2(x_k,u_k)\\
%          &+\mathcal{K}_{u} \psi_3(u_k) +\mathcal{W}_k \Tilde{k}_{w}\nonumber \\
%         \Tilde{k}_w &=[k_{w_1} \quad k_{w_2} \cdots k_{w_n}]\\
%          k_{w_i} &\in \{0,1\} \quad \forall i \in \{1,2,...n\}\\
%         \mathbbm{1}^T \Tilde{k}_{w} &=N_{actuators}\nonumber
%     \end{split}
% \end{equation}

% \end{comment}

==> theorems/not_used_theorems/_rejected_theorems.tex <==
% ==================================================
% NEURAL NETWORK RELATED THEOREMS
% ==================================================
\begin{theorem}
Given a nonlinear system of the form 
\[
x_{k+1} = f(x_k),
\]
where $x \in \mathbb{R}^n$ and $f$ is continuous, if $f$ is approximated by a linear combination of RELU functions of affine transformed state $x$
\[
\Tilde{x}_{k+1} = \Tilde{f}(x_k) \approx \sum_{i=0}^Nw_i\sigma_{a_i,b_i}(x_k) 
\]
such that as $N\rightarrow \infty$, $\Tilde{f}\rightarrow f$ and $\epsilon \rightarrow 0$ where
\begin{equation*}
    \sigma_i(x) = \sigma_{a_i,b_i}(x) = 
    \begin{cases}
        1 &, i=0\\
        max(a_i^Tx+b_i,0) &,i \in {1,2,3,...}
    \end{cases}    
\end{equation*}
is the RELU function with $a_i \in \mathbb{R}^{1\times n}, b_i\in \mathbb{R} \text{ and } w_i \in \mathbb{R}^{n\times1}$, then there exists a linear transformation between $\{\sigma_{a_i,b_i}(x_{k+1})\}$ and $\{\sigma_{a_i,b_i}(x_{k})\}$ with $i \in {0,1,2,...,N}$ with $N\rightarrow \infty$
\[
\psi(x_{k+1}) = K \psi(x_k)
\]
where 
\[
\psi(x) = 
\begin{bmatrix}
 x^T & \sigma_{a_0,b_0} & \sigma_{a_1,b_1}(x) & \sigma_{a_2,b_2}(x) & \cdots
\end{bmatrix}^T
\]
with $a_0 = 0$ and $b_0 = 1$.
\end{theorem}

\begin{proof}

We consider the individual terms of the lifted state $\psi(x_{k+1})$ at time point $k+1$. The first term $x_{k+1}$ is given directly by the approximation of a continuous function using a single hidden layer of RELU networks
\[
\begin{bmatrix}
    x_{k+1}\\
    \sigma_0(x_{k+1})
\end{bmatrix}
= 
\begin{bmatrix}
    0 & w_0 & w_1 & \cdots & w_N\\
    0 & 1 & 0 & \cdots & 0
\end{bmatrix}
\begin{bmatrix}
    x_k\\
    \sigma_0(x_k)\\
    \sigma_1(x_k)\\
    \vdots\\
    \sigma_N(x_k)
\end{bmatrix}
\]
The next term is a DC term which by definition has the property
\[
\sigma_0(x_{k+1}) = \sigma_0(x_k) = 
\begin{bmatrix}
    0 & 1 & 0 & \cdots & 0
\end{bmatrix}
\begin{bmatrix}
    x_k\\
    \sigma_0(x_k)\\
    \sigma_1(x_k)\\
    \vdots\\
    \sigma_N(x_k)
\end{bmatrix}
\]
The rest of the terms are represented generically as $\sigma_i(x_{k+1})$
\begin{align*}
    \sigma_i(x_{k+1}) & = max(a_i^Tx_{k+1} + b_i,0)\\
                      & = max\Bigg{(}\sum_{j=0}^N a_i^Tw_j\sigma_j(x_k) + b_i,0\Bigg{)}\\
                      & = max\Bigg{(}\sum_{j=0}^N \alpha_{ij}\sigma_j(x_k),0\Bigg{)}
\end{align*}        
where $\alpha_{ij} \in \mathbb{R}$ such that
\[
\alpha_{ij} = 
\begin{cases}
a_i^Tw_0 + b_i &,j=0\\
a_iTw_j &,j \in \{1,2,\hdots,N\}
\end{cases} \in \mathbb{R} .
\]
\newpage.
\textbf{Properties of max functions:}
\begin{align*}
    \max(a^Tx+b,0) & = \frac{a^Tx+b + |a^Tx+b|}{2} \\
    \max(a^Tx+b,0) & = (a^Tx+b)u(a^Tx+b) \\
    \max(a,b) \pm c &= \max(a\pm c,b\pm c)\\
    c\max(a,b) &=\max(ca,cb) \text{ if } c\geq0\\
    \max(a,b) + \max(-a,-b) &= |a-b|\\
    \max(a,b) - \max(-a,-b) &= a+b
\end{align*}
\newpage
\textcolor{red}{\textbf{BIG QUESTION} - Does $max\Bigg{(}\sum_{j=0}^N \alpha_{ij}\sigma_j(x_k),0\Bigg{)}$ as a linear combination of the functions
\begin{itemize}
    \item Best case: $\{\sigma_0(x_k),\sigma_1(x_k),\hdots,\sigma_N(x_k)\}$
    \item Second case: $\{\sigma_0(x_k),\sigma_{c_1,d_1}(x_k),\hdots,\sigma_{c_N,d_N}(x_k)\}$
    \item Weak condition: Call $max\Bigg{(}\sum_{j=0}^N \alpha_{ij}\sigma_j(x_k),0\Bigg{)}$ a different RELU function
\end{itemize}}

\textbf{Approach 1: Using properties of max functions}
\begin{align*}
    \sigma_i(x_{k+1}) & =max\Bigg{(}\sum_{j=0}^N \alpha_{ij}\sigma_j(x_k),0\Bigg{)} \\
    &= max\Bigg{(}\sum_{j=0}^N \alpha_{ij}^+\sigma_j(x_k)- \sum_{j=0}^N \alpha_{ij}^-\sigma_j(x_k),0\Bigg{)}\\
    \sigma_i(x_{k+1}) &= max(max(a^Tx+b,0)-max(c^Tx+d,0),0)\\
    &= max(max(a^Tx+b,0),max(c^Tx+d,0)) - max(c^Tx+d)
\end{align*}
\textcolor{violet}{
\textbf{Objective is to show that at least one of these functions are a summation of finite ReLU functions of affine transformed x:}
\begin{align*}
    \sum_{i=1}^M\alpha_i\max(a_i^Tx+b_i,0) + \alpha_0 \stackrel{?}{=} 
    \begin{cases}
        max(max(a^Tx+b,0)-max(c^Tx+d,0),0)\\
        max(max(a^Tx+b,0),max(c^Tx+d,0))\\
        |max(a^Tx+b,0)-max(c^Tx+d,0)|
    \end{cases}
\end{align*}
\textbf{Processing $J = max(max(a^Tx+b,0),max(c^Tx+d,0))$:}
Found a property from one paper
\[
max\{f(x),g(x),h(x)\} = max\{f(x),g(x)\} + max\{f(x),h(x)\} - max\{f(x),min\{g(x),h(x)\}\} 
\]
By substituting
\begin{align*}
    f(x) &= 0\\
    g(x) &= a^Tx+b\\
    h(x) &= c^Tx+d
\end{align*}
we get
\begin{align*}
    \max(\max(a^Tx+b,0),\max(c^Tx+d,0)) &= \max(a^Tx+b,c^Tx+d,0)\\
    = \max(a^Tx+b,0) + \max(c^Tx+d,0) &- \max\{0,\min(a^Tx+b,c^Tx+d)\}
\end{align*}
\textbf{Stuck on: }$\max\{0,\min(a^Tx+b,c^Tx+d)\}$\\
\textbf{Other method:}
\[
max(a,b) = \frac{a+b}{2} + \frac{|a-b|}{2}
\]
Using this to our case yields
\[
\max(\max(a^Tx+b,0),\max(c^Tx+d,0)) = \frac{\max(a^Tx+b,0)+\max(c^Tx+d,0)}{2} + \frac{|\max(a^Tx+b,0)-\max(c^Tx+d,0)|}{2}
\]
\textbf{Stuck on: $|\max(a^Tx+b,0)-\max(c^Tx+d,0)|$}
}\\


where\\
Visual proof that  $max(max(a^Tx+b,0),max(c^Tx+d,0))$ is a summation of RELUs in 1D
\[
\alpha_{ij}^+ = \begin{cases}
\alpha_{ij} &,\alpha_{ij} \geq0\\
0 &,\alpha_{ij}<0
\end{cases} \quad
\alpha_{ij}^- = \begin{cases}
0 &,\alpha_{ij} \geq0\\
-\alpha_{ij} &,\alpha_{ij}<0
\end{cases}
\]
Now, we can define
\[
p(x) \triangleq \sum_{j=0}^N \alpha_{ij}^+\sigma_j(x) \quad q(x) \triangleq  \sum_{j=0}^N \alpha_{ij}^-\sigma_j(x) 
\]
where $p(x)$ and $q(x)$ are positive definite functions. Then
\begin{align*}
    \sigma_i(x_{k+1}) & = max(p(x_k)-q(x_k),0)\\
                      & = max(p(x_k),q(x_k)) -q(x_k)
\end{align*}
\begin{itemize}
    \item We can try $\sigma_{-i}(x_{k+1})$
    \begin{align*}
        \sigma_{-i}(x_{k+1}) &= max(-a_i^Tx_{k+1}-b_i,0)\\
        & = max(-p(x_k)+q(x_k),0)\\
        & = max(p(x_k),q(x_k)) - p(x_k)
    \end{align*}
    With that, we can say
    \[
    \sigma_i(x_{k+1}) -\sigma_{-i}(x_{k+1}) = p(x_k) - q(x(x_k))
    \]
    But
    \begin{align*}
        \sigma_i(x_{k+1}) &= \frac{a_i^Tx_{k+1}+ b_i + |a_i^Tx_{k+1}+ b_i |}{2}\\
        \sigma_{-1}(x_{k+1}) &= \frac{-a_i^Tx_{k+1}- b_i + |a_i^Tx_{k+1}+ b_i |}{2}\\
        \sigma_i(x_{k+1}) -\sigma_{-i}(x_{k+1}) &= a_i^Tx_{k+1}+ b_i = max(a^Tx+b,0) -max(c^Tx+d,0)\\
        \sigma_i(x_{k+1}) +\sigma_{-i}(x_{k+1}) &= |a_i^Tx_{k+1}+ b_i|
    \end{align*}
    The modulus splits the cases
    \item 
\end{itemize}

\end{proof}
% ==================================================
% OUTPUT RELATED THEOREMS
% ==================================================
\textcolor{blue}{
\textbf{Shara's Notes:} This should be a corollary to Theorem 1. There isn't much of a proof that happens here.}
\begin{theorem}
Given the nonlinear system \begin{equation}\begin{aligned} x_{k+1}&=f(x) \\ y_k &= h(x_k)\end{aligned}\end{equation} and a corresponding Koopman observable $\psi:{\cal M}_{\psi} \rightarrow {\cal M}_\psi$ with associated discrete-time Koopman equation  
\begin{equation}
    \psi_x(x_{t+1}) = {\cal K}_x \psi_x(x_{t})
    \end{equation}
and $y \in \text{span}\{ \psi_1, ..., \psi_{n_L}\},$
then any output trajectory $y(t,x_0)$ lies in the image of the Koopman observability matrix 
\begin{equation}
\begin{bmatrix}
 W_h \\ W_h K_x \\  \vdots \\ W_h K_x^t
\end{bmatrix}
\end{equation}
\end{theorem}



\begin{proof}
For any time $k\in \mathbb{Z}_{> 0}$, we have
\begin{equation*}
    \begin{aligned}
        y_k &= W_h\psi(x_k)\\
        y_{k+1} &= W_h\psi(x_{k+1}) = W_h {\cal K}\psi(x_k)\\
        &\vdots\\
        y_{k+\tau} &= W_h\psi(x_{k+\tau}) = W_h {\cal K}^\tau \psi(x_k)
    \end{aligned}
\end{equation*}
and concatenating all of the $\tau + 1$ equations, we get
\begin{equation*}
    y(\tau,x_k) = 
    \begin{bmatrix}
        y_k\\
        y_{k+1}\\
        \vdots\\
        y_{k+\tau}
    \end{bmatrix}=
    \begin{bmatrix}
        W_h\\
        W_h {\cal K}\\
        \vdots\\
        W_h {\cal K}^\tau
    \end{bmatrix}\psi(x_k)
\end{equation*}
Hence, $y(\tau,x_k)$ lies in the span of $\mathcal{O}_{\cal K}(\tau) = \begin{bmatrix}
        W_h^T & (W_h {\cal K})^T & \cdots & (W_h {\cal K}^\tau)^T \end{bmatrix}^T$.
Hence the proof.
\end{proof}   
\textbf{Corollary :}
Assume that for some $\tau$, $\mathcal{O}_{\cal K}(\tau))$ is full column rank, then we can reconstruct the lifted state $\psi(x_k)$, 
\begin{equation}
    \psi(x_k) = \Big{(}\mathcal{O}_{\cal K}^T(\tau)\mathcal{O}_{\cal K}(\tau)\Big{)}^{-1}\mathcal{O}_{\cal K}^T(\tau) y(\tau,x_k)
\end{equation}
Hence, we can derive a state transition matrix purely as form of the outputs
\begin{equation*}
    \begin{aligned}
        &\psi(x_{k+1}) = {\cal K} \psi(x_k)\\
        \Rightarrow &\Big{(}\mathcal{O}_{\cal K}^T(\tau)\mathcal{O}_{\cal K}(\tau)\Big{)}^{-1}\mathcal{O}_{\cal K}^T(\tau) y(\tau,x_{k+1})\\ &= {\cal K}\Big{(}\mathcal{O}_{\cal K}^T(\tau)\mathcal{O}_{\cal K}(\tau)\Big{)}^{-1}\mathcal{O}_{\cal K}^T(\tau) y(\tau,x_k)\\
        \Rightarrow &z_{k+1} = \Tilde{{\cal K}} z_k
    \end{aligned}
\end{equation*}
where
\begin{align*}
    z_k & = \mathcal{O}_{\cal K}^T(\tau) y(\tau,x_k)\\
    \Tilde{{\cal K}} &= \Big{(}\mathcal{O}_{\cal K}^T(\tau)\mathcal{O}_{\cal K}(\tau)\Big{)}{\cal K}\Big{(}\mathcal{O}_{\cal K}^T(\tau)\mathcal{O}_{\cal K}(\tau)\Big{)}^{-1}.
\end{align*}
If $\mathcal{O}_{\cal K}(\tau))$ is diagonal, 
\begin{equation*}
    \begin{aligned}
        \psi(x_{k+1}) &= {\cal K} \psi(x_k)\\
        \Rightarrow y_{k+1} &= \mathcal{O}_{\cal K} {\cal K} \mathcal{O}_{\cal K}^{-1}y_{k}\\
    \end{aligned}
\end{equation*}


\begin{theorem}
Given a nonlinear system with {\it fine-resolution} output equation
\begin{equation}\begin{aligned} x_{t+1}&=f(x_t) \\ y_k &= h(x_\tau^i).\end{aligned}\end{equation} 
Let $\delta_{\tau} =  \tau^{i+1} - \tau^{i}.$ Suppose that the superset of all possible $\Psi$ embeddings is bounded. Then as  $\delta_{\tau} \rightarrow 0$ the space of all feasible Koopman observable subspaces for a fixed $\Psi$ converges to a target embedding space $\Psi_0$, which defines a least element for all $\Psi_{\delta_\tau}$  
\end{theorem}
\begin{proof}
Set up a nested sequence of Koopman operators and function spaces, with decreasing $\delta_\tau$ and show containment is equivalent to a definition of partial order.  Then guarantees monotonicity.  Then argue there is a superset that contains all these Koopman operators and a superset containing all Koopman observables.  Then argue that  because of this, there is a bound on a sequence of sets that is monotonic (defined by partial order of set inclusion), which implies that the sequence of sets has a limit. Use the monotone bounded convergent sequence theorem!!! 
\end{proof}
Can you say something about the approximation error of the true optimal vs. the approximate embedding?



\begin{theorem}
Given a nonlinear system with {\it fine-resolution} output equation
\begin{equation}\begin{aligned} x_{t+1}&=f(x_t) \\ y_t &= h(x_t^i) + \epsilon(t^i).\end{aligned}\end{equation} 00
where $\epsilon(\tau^i) \in E$ and suppose that each element in $E$ is bounded by a least uppper bound $\lambda$.  Then the following optimization problems are equivalent: 
\begin{eqnarray}
&\min_{\Psi} \max_{\epsilon \in E}|| (Y_f-\epsilon) - W_h K\Psi(X_p)||
\end{eqnarray}
and 
\[
\min_{\Psi} || \Psi(X_f) - K\Psi(X_p)|| + \lambda || W_h||
\]
\end{theorem}
\textcolor{red}{\textbf{My thought: The formulation is wrong. The lifted states should be built on y and not on x. Only then can we even think about the error being multiplied with $W_h$ and then have the term $\lambda ||W_h||$ }}

\begin{proof}
\begin{equation*}
    \begin{split}
        &\max_{\epsilon \in E}\min_{K} || \Psi(X_f) - K\Psi(X_p)||\\
        &\text{ subject to \,} Y_p = h(X_p)\\
        = &\max_{\epsilon \in E}\min_{K} || \Psi(X_f) - K\Psi(X_p)|| + M ||Y_p - h(X_p)||\\
        ?= &\min_{K}\max_{\epsilon \in E} || \Psi(X_f) - K\Psi(X_p)|| + M ||Y_p - h(X_p)||\\
        = &\min_{K}[ || \Psi(X_f) - K\Psi(X_p)|| + M \max_{\epsilon \in E}||Y_p - h(X_p)||]\\
        =&\min_{K}[ || \Psi(X_f) - K\Psi(X_p)|| + M \lambda\\
    \end{split}
\end{equation*}
\textcolor{red}{Not sure if this is yielding anything useful or where am I going wrong?}
\end{proof}



% ==================================================
% INPUT RELATED THEOREMS
% ==================================================
\textcolor{blue}{
\textbf{Concerns for Enoch to address:} 
\begin{itemize}
    \item The following theorem doesn't fit well with the rest of the paper
    \item The first half is more like a corollary of the first theorem and also doesn't add value to the work that follows after.
    \item The second half of the theorem seems incorrect and it doesn't tie to the work here because the theorem focuses on output as a state which depends on the observability
\end{itemize}
}

\textbf{Input related theorems: }
\textbf{Theorem: }
Given that a nonlinear system $\dot{x}=f(x,u)\nonumber, x \in \mathbb{R}^n,  u \in \mathbb{R}^m$ has a Koopman operator representation as in (\ref{eq: Koop Final form}), if the $i^{th}$ Koopman state observable is nonlinear $\psi^{(1)}_i(x) \neq x_j \quad \forall j \in \{1,2,...n\}$, then the $i^{th}$ row of the matrix $\mathcal{K}_{u}$ is a zero vector.
% \end{theorem}

\textbf{Proof:}
The system $\dot{x}=f(x,u)$ can be written as
\begin{equation}
    \begin{bmatrix}
        \dot{x}_1\\
        \dot{x}_2\\
        :\\
        \dot{x}_n
    \end{bmatrix} = 
    \begin{bmatrix}
        f_1(x,u)\\
        f_2(x,u)\\
        :\\
        f_n(x,u)
    \end{bmatrix} = 
    \begin{bmatrix}
        f_1^{(1)}(x) + f_1^{(2)}(x,u) + f_1^{(3)}(u)\\
        f_2^{(1)}(x) + f_2^{(2)}(x,u) + f_2^{(3)}(u)\\
        :\\
        f_n^{(1)}(x) + f_n^{(2)}(x,u) + f_n^{(3)}(u)
    \end{bmatrix}\nonumber \\
\end{equation}
has the Koopman representation  in equation (\ref{eq: Koop Final form}) with the observables
\begin{equation}
    \begin{split}
        \psi^{(1)}_i(x)&:\mathbb{R}^{n\times1} \rightarrow \mathbb{R} \quad i = 1,2,...N\nonumber\\
        \psi^{(2)}_j(x,u)&:\mathbb{R}^{n \times m} \rightarrow \mathbb{R}\quad j = 1,2,...M\nonumber\\
        \psi^{(3)}_k(u)&:\mathbb{R}^{m\times 1} \rightarrow \mathbb{R}\quad k = 1,2,...P\nonumber
    \end{split}
\end{equation}
can be written as
\begin{equation}
    \scalebox{0.80}{
    \begin{bmatrix}
        \dot{\psi}_1^{(1)}\\
        \dot{\psi}_2^{(1)}\\
        :\\
        \dot{\psi}_N^{(1)}
    \end{bmatrix} = 
    \begin{bmatrix}
        k_{x1}^T\\
        k_{x2}^T\\
        :\\
        k_{xN}^T
    \end{bmatrix}
    \begin{bmatrix}
        \psi_1^{(1)}\\
        \psi_2^{(1)}\\
        :\\
        \psi_N^{(1)}
    \end{bmatrix}+
    \begin{bmatrix}
        k_{xu1}^T\\
        k_{xu2}^T\\
        :\\
        k_{xuM}^T
    \end{bmatrix}
    \begin{bmatrix}
        \psi_1^{(2)}\\
        \psi_2^{(2)}\\
        :\\
        \psi_M^{(2)}
    \end{bmatrix}+
    \begin{bmatrix}
        k_{u1}^T\\
        k_{u2}^T\\
        :\\
        k_{uP}^T
    \end{bmatrix}
    \begin{bmatrix}
        \psi_1^{(3)}\\
        \psi_2^{(3)}\\
        :\\
        \psi_P^{(3)}
    \end{bmatrix}}\label{eq: Koop_input complete matrix} \\
\end{equation}
We construct a map between the nonlinear system and the Koopman system
\begin{equation}
    \begin{split}
        \dot{\psi}^{(1)}_i(x) &= \sum_{j=1}^n\frac{\partial \psi^{(1)}_i(x)}{\partial x_j}\dot{x}_j\\
        &= \sum_{j=1}^n\frac{\partial \psi^{(1)}_i(x)}{\partial x_j}\Big{(}f_j^{(1)}(x) + f_j^{(2)}(x,u) + f_j^{(3)}(u) \Big{)}
    \end{split}
    \label{eq: NLsys differentiated}
\end{equation}
Comparing the equations (\ref{eq: Koop_input complete matrix}) and (\ref{eq: NLsys differentiated}), separating out the terms that are purely functions of $x$ yields
\begin{equation}
    k_{xi}^T\psi^{(1)} (x) = \sum_{j=1}^n\frac{\partial \psi^{(1)}_i (x)}{\partial x_j}\Big{(}f_j^{(1)}(x)  \Big{)} \nonumber
\end{equation}
\begin{itemize}
    \item \textbf{Case 1:} $\psi^{(1)}_i(x) \neq a^Tx$  where $a$ is a constant vector.
        \begin{flalign*}
            \begin{split}
                \frac{\partial \psi^{(1)}_i(x)}{\partial x_j}&\neq const \\
                \implies k_{xu_i}^T\psi^{(2)}_i &= \sum_{j=1}^n\frac{\partial \psi^{(1)}_i(x)}{\partial x_j}\Big{(}f_j^{(2)}(x,u) + f_j^{(3)}(u)  \Big{)}\\
                \implies k_{u_i}^T\psi_i^{(3)} &=0
                \nonumber
            \end{split}
        \end{flalign*}
        Since $\psi_i^{(3)}\neq0, \quad k_{u_i}^T=[0 \quad 0\quad  \cdots \quad0]$\\
        \textcolor{red}{Think of observable $\psi_1 = x_1^2$ and dynamics $\dot{x}_1 = \frac{u}{x_1}$. Then, $\partial_t \psi_1 = \partial_{x_1} \psi_1 \frac{u}{x_1} = 2u$ - which should come from $\psi^{(3)}$.}
    \item \textbf{Case 2:} $\psi^{(1)}_i(x) = a^Tx$  where $a$ is a constant vector.
    \begin{flalign*}
        \begin{split}
            \frac{\partial \psi^{(1)}_i(x)}{\partial x_j}&= a^T \\
            \implies k_{xu_i}^T\psi^{(2)}_i &= \sum_{j=1}^n a^Tf_j^{(2)}(x,u)\\
            \text{and }\quad k_{u_i}^T\psi_i^{(3)} &=\sum_{j=1}^n a^Tf_j^{(3)}(u)\\
            \implies k_{u_i}^T&\neq[0 \quad 0\quad  \cdots \quad0]
            \nonumber
        \end{split}
    \end{flalign*}
\end{itemize}
Therefore, if the Koopman state observable is nonlinear, then the corresponding row in the pure input matrix $\mathcal{K}_u$ is equal to $[0 \quad 0\quad  \cdots \quad0]$.

\textbf{Corollary:} If the dictionary of observables is state inclusive, this yields a structure of $\mathcal{K}_u$ as follows:
\begin{equation}
    \begin{bmatrix}
        \psi^{(1)}_1\\
        :\\
        \psi^{(1)}_n\\
        \psi^{(1)}_{n+1}\\
        :\\
        \psi^{(1)}_N
    \end{bmatrix} =
    \begin{bmatrix}
        x_1\\

        :\\
        x_n\\
        \psi^{(1)}_{n+1}\\
        :\\
        \psi^{(1)}_N
    \end{bmatrix} \implies \mathcal{K}_u =
    \begin{bmatrix}
        k_{u1}^T\\
        :\\
        k_{un}^T\\
        k_{u(n+1)}^T\\
        :\\
        k_{uP}^T
    \end{bmatrix}=
    \begin{bmatrix}
        k_{u1}^T\\
        :\\
        k_{un}^T\\
        0\\
        :\\
        0
    \end{bmatrix}\nonumber
\end{equation}

\begin{theorem}
If the inputs $w_1$ and $w_2$ affect the dynamics of the nonlinear system $\dot{x} = \Tilde{f}(x,u,w_1,w_2)$ independently as given by
\begin{equation}
    \dot{x} = \Tilde{f}(x,u,w_1,w_2)=f(x,u) + g_1(x,u,w_1) + g_2(x,u,w_2)\nonumber
\end{equation}
then the inputs affect the dynamics of the Koopman lifted system independently
\begin{equation*}
    \begin{split}
        \dot{\psi}^{(1)}(x) &= \Tilde{\mathcal{K}}_{xu} \Tilde{\psi}^{(1)}(x,u)+\sum_{k=i}^q k_{w_i}\Tilde{\mathcal{K}}_{xuw_i} \Tilde{\psi}^{(i)}(x,u,w_i)
    \end{split} 
\end{equation*}
where
\begin{equation}
    \begin{split}
        \Tilde{\mathcal{K}}_{xu} &= [\mathcal{K}_{x} \quad \mathcal{K}_{xu} \quad \mathcal{K}_{u} ]\\
        \Tilde{\mathcal{K}}_{xuw_i} &= [\mathcal{K}_{w_i} \quad \mathcal{K}_{xw_i}  \quad \mathcal{K}_{uw_i} \quad \mathcal{K}_{xuw_i} ]\\
        \Tilde{\psi}^{(1)}(x,u) &= 
        \scalebox{0.85}{
        \begin{bmatrix}
        \psi^{(1)}(x) \\
        \psi^{(2)}(x,u) \\
        \psi^{(3)}(u)
        \end{bmatrix} }
        \Tilde{\psi}^{(i)}(x,u,w_i) = 
        \scalebox{0.85}{
        \begin{bmatrix}
        \psi^{(i4)}(w_i) \\
        \psi^{(i5)}(x,w_i) \\
        \psi^{(i6)}(u,w_i)\\
        \psi^{(i7)}(x,u,w_i)
        \end{bmatrix}}\nonumber
    \end{split} 
\end{equation}
\end{theorem}

\textbf{Proof:}
Since the inputs $w_1$ and $w_2$ affect the dynamics of the system independently, we can decompose our nonlinear system as 
\begin{equation}
    \dot{x} = \Tilde{f}(x,u,w_1,w_2)=f(x,u) + g_1(x,u,w_1) + g_2(x,u,w_2)\nonumber
\end{equation}
Suppose $\psi_i^{(1)}(x):\mathbb{R}^n\rightarrow \mathbb{R} \quad \forall \quad i \in \{1,2,...N\}$ is used to construct the Koopman observable as in (\ref{eq: Koop Final form}), then 
\begin{equation}
    \begin{split}
        \dot{\psi}^{(1)}(x) = \mathcal{K}_{x} \psi^{(1)}(x) &+ \mathcal{K}_{xuw_1w_2} \Tilde{\psi}^{(2)}(x,u,w_1,w_2)\\ 
        &+ \mathcal{K}_{uw_1w_2} \Tilde{\psi}^{(3)}(u,w_1,w_2) \nonumber \\
    \end{split}
\end{equation}
represents the Koopman system which can be rewritten as 
\begin{equation}
    \begin{split}
        \dot{\psi}^{(1)}(x) = \mathcal{K}_{x} \psi^{(1)}(x) + \mathcal{K}_{xu} \psi^{(2)}(x,u) + \mathcal{K}_{u} \psi^{(3)}(u) \\
        + \mathcal{K}_{w_1} \psi^{(4)}(w_1)  + \mathcal{K}_{w_2} \psi^{(5)}(w_2) + \mathcal{K}_{xw_1} \psi^{(6)}(x,w_1)\\
        + \mathcal{K}_{xw_2} \psi^{(7)}(x,w_2)+ \mathcal{K}_{uw_1} \psi^{(8)}(u,w_1)+ \mathcal{K}_{uw_2} \psi^{(9)}(u,w_2)\\
        + \mathcal{K}_{w_1w_2} \psi^{(10)}(w_1,w_2)+ \mathcal{K}_{xuw_1} \psi^{(11)}(x,u,w_1)\\
        + \mathcal{K}_{xuw_2} \psi^{(12)}(x,u,w_2)  + \mathcal{K}_{xw_1w_2} \psi^{(13)}(x,w_1,w_2)\\
        + \mathcal{K}_{uw_1w_2} \psi^{(14)}(u,w_1,w_2) + \mathcal{K}_{xuw_1w_2} \psi^{(15)}(x,u,w_1,w_2)\nonumber \\
    \end{split}
\end{equation}
But, from the nonlinear differential equation, it can be seen that
\begin{equation}
    \begin{split}
        &\dot{\psi}^{(1)}(x) = \sum_{j=1}^n\frac{\partial \psi^{(1)}(x)}{\partial x_j}\dot{x}_j\\
        &= \nabla_x^T(\psi^{(1)}(x))\Big{(}f(x,u) + g_1(x,u,w_1) + g_2(x,u,w_2)\Big{)}\nonumber
    \end{split}
\end{equation}
By comparing the terms in the original space and the Koopman space 
\begin{equation}
    \begin{split}
        \nabla_x^T(\psi^{(1)}(x))f= \mathcal{K}_{x} \psi^{(1)}(x) + \mathcal{K}_{xu} \psi^{(2)}(x,u) + \mathcal{K}_{u} \psi^{(3)}(u)\\
        \nabla_x^T(\psi^{(1)}(x))g_1=\mathcal{K}_{w_1} \psi^{(4)}(w_1)+ \mathcal{K}_{xw_1} \psi^{(6)}(x,w_1)\\
        + \mathcal{K}_{uw_1} \psi^{(8)}(u,w_1)+ \mathcal{K}_{xuw_1} \psi^{(11)}(x,u,w_1)\\
        \nabla_x^T(\psi^{(1)}(x))g_2=\mathcal{K}_{w_2} \psi^{(5)}(w_2)+ \mathcal{K}_{xw_2} \psi^{(7)}(x,w_2)\\
        + \mathcal{K}_{uw_2} \psi^{(9)}(u,w_2) + \mathcal{K}_{xuw_2} \psi^{(12)}(x,u,w_2)\nonumber
    \end{split}
\end{equation}
The remaining terms must go to zero and since the observables cannot become zero, the matrices are forced to zero
\begin{equation}
    \mathcal{K}_{w_1w_2}=0 \quad \mathcal{K}_{xw_1w_2}=0 \quad \mathcal{K}_{uw_1w_2}=0 \quad \mathcal{K}_{xuw_1w_2}=0 \nonumber
\end{equation}
Hence the Koopman space equation can be written as
\begin{equation}
    \begin{split}
            \dot{\psi}^{(1)}(x) = [\mathcal{K}_{x} \quad \mathcal{K}_{xu} \quad \mathcal{K}_{u} ]
        \begin{bmatrix}
        \psi^{(1)}(x) \\
        \psi^{(2)}(x,u) \\
        \psi^{(3)}(u)
        \end{bmatrix}\\
        +[\mathcal{K}_{w_1} \quad \mathcal{K}_{xw_1}  \quad \mathcal{K}_{uw_1} \quad \mathcal{K}_{xuw_1} ]
        \begin{bmatrix}
        \psi^{(4)}(w_1) \\
        \psi^{(6)}(x,w_1) \\
        \psi^{(8)}(u,w_1)\\
        \psi^{(11)}(x,u,w_1)
        \end{bmatrix}\\
        +[\mathcal{K}_{w_2} \quad \mathcal{K}_{xw_2}  \quad \mathcal{K}_{uw_2} \quad \mathcal{K}_{xuw_2} ]
        \begin{bmatrix}
        \psi^{(5)}(w_2) \\
        \psi^{(7)}(x,w_2) \\
        \psi^{(9)}(u,w_2)\\
        \psi^{(12)}(x,u,w_2)
        \end{bmatrix}\\
    \end{split} \label{eq: Koop dual input w_1 w_2}
\end{equation}
Hence the inputs $w_1$ and $w_2$ affect the dynamics of the Koopman system independently.

We can generalize the system (\ref{eq: Koop dual input w_1 w_2}) to $q$ new inputs along with the actuator admissibility vector $\Tilde{k}_w$ as
\begin{equation}
    \begin{split}
        \dot{\psi}^{(1)}(x) &= \Tilde{\mathcal{K}}_{xu} \Tilde{\psi}^{(1)}(x,u)\\
        &+\sum_{k=i}^q k_{w_i}\Tilde{\mathcal{K}}_{xuw_i} \Tilde{\psi}^{(i)}(x,u,w_i)
    \end{split} \label{eq: Koop multi input}
\end{equation}
where
\begin{equation}
    \begin{split}
        \Tilde{\mathcal{K}}_{xu} &= [\mathcal{K}_{x} \quad \mathcal{K}_{xu} \quad \mathcal{K}_{u} ]\\
        \Tilde{\mathcal{K}}_{xuw_i} &= [\mathcal{K}_{w_i} \quad \mathcal{K}_{xw_i}  \quad \mathcal{K}_{uw_i} \quad \mathcal{K}_{xuw_i} ]\\
        \Tilde{\psi}^{(1)}(x,u) &= 
        \scalebox{0.85}{
        \begin{bmatrix}
        \psi^{(1)}(x) \\
        \psi^{(2)}(x,u) \\
        \psi^{(3)}(u)
        \end{bmatrix} }
        \Tilde{\psi}^{(i)}(x,u,w_i) = 
        \scalebox{0.85}{
        \begin{bmatrix}
        \psi^{(i4)}(w_i) \\
        \psi^{(i5)}(x,w_i) \\
        \psi^{(i6)}(u,w_i)\\
        \psi^{(i7)}(x,u,w_i)
        \end{bmatrix}}\nonumber
    \end{split} 
\end{equation}

==> theorems/not_used_theorems/theorem_linear_dynamics_nonlinear_output.tex <==

\textcolor{blue}{\textbf{Why this theorem?} This theorem is more of an example for what solution does the oc-deepDMD finds for a linear system with outputs spanned by polynomials.}
\textcolor{red}{\textbf{Question:} Should this still be written as a theorem or as an illustration for the concept?}
\begin{theorem}
Given a finite-dimensional linear time-invariant dynamical system 
\[x_{t+1} = Ax_t \]
and nonlinear scalar output equation 
\[y = D(x_t) \]
where  \[D = \begin{bmatrix} p_1(x) & p_2(x) & \hdots & p_{N_D}(x)\end{bmatrix}^T \in \mathbb{R}^{N_D}\],
then the state-inclusive output lifting $\psi = (x, D(x))\in\mathbb{R}^{N_D+n}$ is a Koopman observable with Koopman equation 
\[
\psi(x_{t+1}) = K \psi(x_t) 
\]
where 
$K = \begin{bmatrix} A & 0  \\ 0 & C_D \end{bmatrix}$
and $C_D$ is a coefficient matrix defined by the scalar weighting terms in $D$ and $A.$
\end{theorem}
% \newpage
\begin{proof}
Write out each polynomial as a weighted combination of multinomial of xs and then book keep. And use linearity (twice). 
\[
p_i(x) = \sum_{j=1}^\infty \alpha_j x_1^{p_{ij1}}x_2^{p_{ij2}}\hdots x_n^{p_{ijn}} + \alpha_{ij0}
\]
Define $p_i(x) = \Big{\{}\prod\limits_{j=1}^n (x(j))^{n_{i,j}}| \sum\limits_{j=1}^n n_{i,j} = i\Big{\}}$ be the set of all monomials of order $i$ where $x(j)$ is the $j^{th}$ element of the vector $x$. Any element of the set $p_i(x_{k+1})$ can be written as
\begin{align*}
    &\prod_{j=1}^n (x_{k+1}(j))^{n_{i,j}}\\
    &= \prod_{j=1}^n \sum_{\substack{k_{j1}+k_{j2}+\\\cdots+k_{jn} = n_{i,j}}} {\binom{n_{i,j}}{k_{j1},k_{j2},\cdots,k_{jn}}} \prod_{q=1}^n (a_{jq})^{k_{jq}} (x_{k}(q))^{k_{jq}}\\
    &= \sum_{\substack{k_{11}+k_{12}+\\\cdots+k_{1n} = n_{i,1}}} \sum_{\substack{k_{21}+k_{22}+\\\cdots+k_{2n} = n_{i,2}}}\cdots \sum_{\substack{k_{n1}+k_{n2}+\\\cdots+k_{nn} = n_{i,n}}} \prod_{j=1}^n\prod_{q=1}^n(x_{k}(q))^{k_{jq}}
\end{align*}
where
\[
\alpha_\Bigg{(}\prod_{j=1}^n {\binom{n_{i,j}}{k_{j1},k_{j2},\cdots,k_{jn}}} \prod_{q=1}^n (a_{jq})^{k_{jq}}\Bigg{)}
\]

We can show that all elements of $p_i(x_{k+1})$ can be written as a linear combination of the elements in the set $p_i(x_k)$
\end{proof}


==> theorems/not_used_theorems/theorem_sampling_system_output_different.tex <==

\begin{theorem}
Given a nonlinear system with a finer-resolution output equation
\begin{align} 
    x((p+1)N_sT_s) = x_{p+1}&=f(x_p) = f(x(pN_sT_s)) \nonumber \\
    y(qT_s) = y_q &= h(x_q) = h(x(qT_s)) \nonumber
\end{align}
where  $N_s \in \mathbb{Z}_{>0}$ is the ratio of the sampling rates of state to output, we can construct a Koopman operator for the concatenated output of all outputs between two instances of the coarser resolution.
\end{theorem}

\begin{proof}
We consider the finer resolution system dynamics $x_{q+1}=f(x_q)$ with finer resolution output equation $y_q = h(x_q)$ to have a Koopman operator representation given by 
\begin{align*}
    \psi(x_{q+1}) &= K_q\psi(x_q) \\ 
        y_q &= W_{hq}\psi(x_q)
\end{align*} 
Now, we reformulate the state in the coarser resolution 
\begin{align*}
    &x_{p+1} = x(pN_sT_s + N_sT_s) = \underbrace{f\circ f \circ \cdots \circ f}_{N_s \hspace{1pt} times}(x(pN_sT_s)) \\
    &\Rightarrow \psi(x_{p+1}) = K_q^{N_s}\psi(x_p)
\end{align*}
Now, we formulate the output in the coarser resolution by concatenating all the outputs between two time points in the coarser resolution
\begin{align*}
    z_p = 
    \begin{bmatrix}
        y(pN_sT_s)\\
        y(pN_sT_s + Ts)\\
        \vdots\\
        y((p+1)N_sT_s -1)\\
    \end{bmatrix}&=
    \begin{bmatrix}
        W_h\\
        W_h K\\
        \vdots\\
        W_h K^{N_s-1}
    \end{bmatrix}\psi(x_p)\\
    z_p &= W_{hp} \psi(x_p)
\end{align*}

\end{proof}

% === ============================================================
% END OF PROOF






% EVERYTHING IS IS THE PROOF FROM BEFORE

\begin{comment}


Let's define the state at a generic discrete time instant $k$ to be given by 
$x_k = x(kT_s)$ where $T_s$ is the sampling time of the continuous state given by $x(t)$. Since $p=N_sq$ where $N_s \in \mathbb{Z}_{\geq0}$, time scale $q$ samples the state at a finer resolution than time scale $p$. Since $f$ is analytic, by theorem \ref{theorem: existence of Kx and Wh}, we know that a Koopman operator exists for the system 
\begin{equation*}
    \begin{aligned} 
        x_{q+1}&=f(x_q) \\ 
        y_q &= h(x_q)
    \end{aligned}
\end{equation*}
and is given by 
\begin{equation*}
    \begin{aligned} 
        \psi(x_{q+1}) &= K\psi(x_q) \\ 
        y_q &= W_h\psi(x_q)
    \end{aligned}
\end{equation*}
Now, if the state equation is constructed for a coarser system given by 
\begin{equation*}
        x_{p+1}=x_{N_sq+N_s} = \underbrace{f\circ f \circ \cdots \circ f}_{N_s \hspace{1pt} times}(x_{N_sq}) 
\end{equation*}
So, the Koopman operator with the output equation becomes
\begin{equation*}
    \begin{aligned} 
        \psi(x_{p+1}) &= \tilde{K}\psi(x_{p})\\
        y_p &= W_h\psi(x_p)
    \end{aligned}
\end{equation*}
where $\tilde{K} = K^{N_s}$.

Furthermore, we can construct a new state $z_p$ given by the accumulation of all the output measurements between the two sampling instances in the time scale of $p$ given by
\begin{equation*}
    z_p = 
    \begin{bmatrix}
        y_{_{N q}}\\
        y_{_{N q+1}}\\
        \vdots\\
        y_{_{N(q+1)-1}}
    \end{bmatrix}=
    \begin{bmatrix}
        W_h\\
        W_h K\\
        \vdots\\
        W_h K^{N_s-1}
    \end{bmatrix}x_{_{N q}} = \tilde{W}_h x_p.
\end{equation*}
Hence, we can construct a new Koopman system with all the possible measurements by the collective equation
\begin{equation*}
    \begin{aligned} 
        \psi(x_{p+1}) &= \tilde{K}\psi(x_{p})\\
        z_p &= \tilde{W}_h\psi(x_p)
    \end{aligned}
\end{equation*}
Therefore, we have proved that if a Koopman operator exists for a fine resolution system, a Koopman operator exists for the coarser resolution system 
\end{comment}

==> theorems/not_used_theorems/wrong_theorems/wrong_theorem_1.tex <==
\begin{theorem}
Given the nonlinear system 
\begin{equation*}
    \begin{split}
        \dot{x} &= f(x)\\
        y &= h(x) 
    \end{split}
\end{equation*}with $f:\mathcal{M}\rightarrow \mathcal{M} $ and $h:\mathcal{M}\rightarrow \mathbb{R}^p $, if $f(x)$ and $h(x)$ are $C^{N_d} [0,\infty)$ differentiable with $N_d=\infty$ or $f(x)$ and $h(x)$ have a finite Taylor series expansion, then there exists a Koopman generator  $\mathcal{K}$ for the above nonlinear system with observables $\psi(x):\mathcal{M} \rightarrow \mathbb{R}^N$ defined by 
\begin{equation*}
    \dot{\psi}(x) = \mathcal{K}\psi(x),
\end{equation*}
such that $h(x) \in span\{\psi(x)\}$ and allows us to write the output equation for the Koopman system as
\begin{equation*}
    y = W_h\psi(x).
\end{equation*}
\end{theorem}
\textcolor{red}{For the proofs, the direction of approach is wrong and a plausible approach would be to use differential geometry and talk about the lie algebra being the same for the full state observable Koopman system }

\begin{proof}
\textcolor{red}{Alternate proof :} For the nonlinear system
\begin{equation*}
    \begin{split}
        \dot{x} &= f(x)\\
        y &= h(x) 
    \end{split}
\end{equation*}
if $h(x)$ is differentiable, then we can append the state equation with the output dynamics as
\begin{equation*}
    \begin{split}
        \begin{bmatrix}
            \dot{x}\\
            \dot{y}
        \end{bmatrix} = \begin{bmatrix}
            f(x)\\
            \dot{h}(x)
        \end{bmatrix}=\Tilde{f}(x)
    \end{split}
\end{equation*}

If the new vector field $\Tilde{f}(x) =[f^T(x),\dot{h}^T(x)]^T$ is infinitely differentiable, then a Koopman operator exists for the concatenated system. This follows from Lemma 1 in \cite{yeung2018koopmanGramian} that if the function \Tilde{f}(x) is infinitely differentiable, then by Taylor series expansion
\begin{equation*}
    \Tilde{f}(x) = \Tilde{f}(0) + \frac{\partial \Tilde{f}}{\partial x}x + \frac{\partial^2 \Tilde{f}}{\partial x^2}x^2 +\cdots = \mathcal{K}\psi(x)
\end{equation*}
Since $\Tilde{f}$ is only a function of $x$, the Koopman generator for the concatenated system can be written as
\begin{equation*}
    \begin{split}
        \begin{bmatrix}
            \dot{x}\\
            \dot{\varphi}(x)\\
            \dot{y}\\
            \dot{\varphi}(x,y)\\
            \dot{\varphi}(y)
        \end{bmatrix} = 
        \begin{bmatrix}
            K_{11} & K_{12} & 0 & 0 & 0\\
            K_{21} & K_{22} & 0 & 0 & 0\\
            K_{31} & K_{23} & 0 & 0 & 0\\
            0 & 0 & 0 & 0 & 0\\
            0 & 0 & 0 & 0 & 0
        \end{bmatrix}
        \begin{bmatrix}
            x\\
            \varphi(x)\\
            y\\
            \varphi(x,y)\\
            \varphi(y)
        \end{bmatrix}
    \end{split}
\end{equation*}
which is a super set of the Koopman operator for the nonlinear system $\dot{x} = f(x)$ given by
\begin{equation*}
    \begin{split}
        \begin{bmatrix}
            \dot{x}\\
            \dot{\varphi}(x)\\
        \end{bmatrix} = 
        \begin{bmatrix}
            K_{11} & K_{12}\\
            K_{21} & K_{22} 
        \end{bmatrix}
        \begin{bmatrix}
            x\\
            \varphi(x)\\
        \end{bmatrix}
    \end{split}
\end{equation*}
Hence, it has been should that the Koopman system of the state dynamics is a subset of the Koopman system of the state dynamics with output.
\end{proof}

\begin{proof}
\textcolor{red}{Alternate proof is incomplete and I'm sure sure this is the right direction because we need to establish under what conditions can $\varphi^{(2)}(x)$ form a Koopman basis}
Given that the system
\begin{equation*}
    \dot{x} = f(x)\\
\end{equation*}
has a Koopman generator $\mathcal{K}$ for the set of observables $\{x_i\}\bigcup \{\varphi^{(1)}_i(x)\}$ such that
\begin{equation*}
    \begin{bmatrix}
        \dot{x}\\
        \dot{\varphi}^{(1)}(x)
     \end{bmatrix}=
     \begin{bmatrix}
        K_{11} & K_{12}\\
        K_{21} & K_{22}
     \end{bmatrix}
     \begin{bmatrix}
        x\\
        \varphi^{(1)}(x)
     \end{bmatrix}
\end{equation*}
and that the output function $y \in span\{x,\varphi^{(1)}(x),\Tilde{\varphi}^{(2)}(x)\}$, then, we can construct an extended list of observables $\varphi^{(2)}(x) \text{ such that} \Tilde{\varphi}^{(2)}(x) \subset \varphi^{(2)}(x)$ 
\begin{equation*}
    \begin{split}
        \begin{bmatrix}
            \dot{x}\\
            \dot{\varphi}^{(1)}(x)\\
            \dot{\varphi}^{(2)}(x)
         \end{bmatrix} &=
         \begin{bmatrix}
            K_{11} & K_{12} & 0\\
            K_{21} & K_{22} & 0\\
            K_{31} & K_{32} & K_{33}
         \end{bmatrix}
         \begin{bmatrix}
            x\\
            \varphi^{(1)}(x)\\
            \varphi^{(2)}(x)
         \end{bmatrix}\\
         y &=
         \begin{bmatrix}
            W_{h0} & W_{h1} & W_{h2} 
         \end{bmatrix}
         \begin{bmatrix}
            x\\
            \varphi^{(1)}(x)\\
            \varphi^{(2)}(x)
         \end{bmatrix}
     \end{split}
\end{equation*}
is the Koopman generator representation for the system
\begin{equation*}
    \begin{split}
        \dot{x} &= f(x,u)\\
        y &= h(x) 
    \end{split}
\end{equation*}
\end{proof}


==> theorems/notes_for_theorem_1.tex <==
\textcolor{ForestGreen}{\textbf{Some notes to watch out in theorem 1}:
For the output functions $h(x) \in \mathbb{R}^p$ and the lifting functions $\psi(x) \in \mathbb{R}^{n_L}$ such that $h(x) = W_h\psi(x)$, 
\begin{itemize}
    \item if we claim $p \geq n_L$, i.e., the number of outputs is greater than the number of inputs, lets take an example to see what happens
    \[
    \begin{bmatrix}
    h_1\\h_2\\h_3
    \end{bmatrix} =
    \begin{bmatrix}
    W_{11} & W_{12}\\
    W_{21} & W_{22}\\
    W_{31} & W_{32}
    \end{bmatrix}
    \begin{bmatrix}
    \psi_1\\ \psi_2
    \end{bmatrix}
    \]
    implying $h_1,h_2,h_3$ cannot be linearly independent
    \item if we claim $p < n_L$, then we have something like
    \[
    \begin{bmatrix}
    h_1\\h_2\\h_3
    \end{bmatrix} =
    \begin{bmatrix}
    W_{11} & W_{12} & W_{13} & W_{14}\\
    W_{21} & W_{22} & W_{23} & W_{24}\\
    W_{31} & W_{32} & W_{33} & W_{34}\\
    W_{41} & W_{42} & W_{43} & W_{44}
    \end{bmatrix}
    \begin{bmatrix}
    \psi_1\\ \psi_2 \\ \psi_3 \\ \psi_4
    \end{bmatrix}
    \]
    \begin{itemize}
        \item not full column rank
        \item and we have $n_L>p$
        \item Since the outputs are linearly independent, the rank of $W_h$ is $p$ 
    \end{itemize}
\end{itemize}
\textbf{Conclusion :} So we can have that either $h(x)$ is linearly independent or  
}

==> theorems/proposition_observability_of_the_KO.tex <==

\begin{prop} \label{theorem: existence of Kx and Wh}
Given the nonlinear system of the form (\ref{eq: nonlinear system with output}), if the functions $f$ and $h$ are real analytic on the open set $\mathcal{M}$, then there exists an OC-KO representation of the form (\ref{eq: Koopman system with output}) in the region of convergence of the Taylor series expansion of $f$ and $h$.
\end{prop}

\begin{pf}
Let us consider a dictionary of polynomial lifting functions 
$
\mathcal{D} = \{\psi_1(x),\psi_2(x),\hdots\}, \quad \psi_r(x)=\displaystyle\prod_{i=1}^n x_i^{p_{r,i}}
$
 where $p_{r,i} \in \mathbb{Z}^+$. Since $f$ is real analytic in $\mathcal{M}$, for any $x_0 \in \mathcal{M}$, there exists a Taylor series expansion centered about $x_0$ that converges to $f(x)$ for a neighborhood of $x_0$. Suppose $f(x) = \begin{bmatrix}f_1(x) & \cdots f_n(x)\end{bmatrix}^T$, the Taylor series expansion of $f$ about $x_0$ yields
\begin{equation*}
    f_i(x) \hspace{-2.5pt}=\hspace{-2.5pt} f_i(x_0) + \frac{\partial f_i}{\partial x}\Bigg{|}_{x_0}x + x^T \frac{\partial^2 f_i}{\partial x^2}\Bigg{|}_{x_0}x + \cdots \hspace{-2.5pt}=\hspace{-2.5pt} \sum_{j=1}^{\infty} c_{ij}\psi_j(x).
\end{equation*}
where each term lies in $\mathcal{D}$. Suppose $x_k= \begin{bmatrix}x_{k,1} & \cdots x_{k,n}\end{bmatrix}^T$  where $x_{k,i}$ indicates the $i^{th}$ state at discrete time index $k$. $x_k$ propagated by one time step yields a linear combination of functions in $\mathcal{D}$ as $x_{k+1,i} = f_i(x) = \sum_{j=1}^{\infty} c_{ij}\psi_j(x_k)$.
To construct a linear system, we propagate each function on the right hand side $\psi_j(x_k)$ by one time step
\begin{equation*}
        \psi_j(x_{k+1}) = \displaystyle\prod_{i=1}^{n} x_{k+1,i}^{p_{j,i}} = \displaystyle\prod_{i=1}^{n} \Big{(}\sum_{j=1}^{\infty} c_{ij}\psi_j(x_k)\Big{)}^{p_{j,i}}
\end{equation*}
Since Lemma \ref{lemma: invariant dictionary} states that the product of any number of functions in $\mathcal{D}$ lies in $\mathcal{D}$, $\psi_j(x_{k+1}) = \sum_{r=1}^{\infty} k_{ir}\psi_r(x_k)$. Concatenating the expressions of $x_{k+1,j}$ and $\psi_j(x_{k+1})$ for all $j$, we get the Koopman representation $\psi(x_{k+1}) = K\psi(x_k)$.

Similarly, for the output equation, we can expand each function $h_i$ in $h(x) = \begin{bmatrix}h_1(x) & h_2(x) & \cdots h_m(x)\end{bmatrix}^T$ using the Taylor series expansion about $x=x_0$ to yield
\begin{equation*}
    \begin{aligned}
       h_i(x) \hspace{-2pt}&= h_i(x_0) \hspace{-2pt}+\hspace{-2pt} \frac{\partial h_i}{\partial x}\Bigg{|}_{x_0} \hspace{-9pt} x + \hspace{-2pt}x^T \frac{\partial^2 h_i}{\partial x^2}\Bigg{|}_{x_0}\hspace{-9pt}x + \cdots = \hspace{-4pt}\sum_{j=1}^{\infty} w_{ij}\psi_j(x)\\
       \Rightarrow y_k& = W_h\psi(x_k)
    \end{aligned}
\end{equation*}
Hence, if $f$ and $h$ of the nonlinear system (\ref{eq: nonlinear system with output}) are analytic in the open set $\mathcal{M}$, a state inclusive OC-KO representation of the form (\ref{eq: Koopman system with output}) exists for that system. 
\hspace*{\fill}~\qed\par
\end{pf}

When outputs partially measure the states, we see that time-delay embedded outputs have a diffeomorphic map with a subspace of the lifting functions under a similarity transform and the dynamics evolving in the two spaces are diffeomorphic conjugate. This theorem is shown only for a finite case and can be easily extended to an infinite case. 

\begin{cor}
Using the arguments similar to 
\end{cor}

\begin{cor}
When $n_o = n_L$, then $z_k$ has a diffeomorphic map with the entire dictionary of observables
\end{cor}


can capture the output dynamics and form a map with the state dynamics in OC-KO. When $n_o=n_L$, the outputs capture the dynamics of the entire lifted state ($\psi(x)$). To fuse the state and output dynamics under a diffeomorphism, we consider 
\begin{itemize}
    \item the observable lifting functions for the state dynamics as only $\psi_o(x)$ lies in the span of the time-delay embedded outputs
    \item projection of the time-delay embedded output for the output dynamics as the dimension of  $\begin{bmatrix} y_k & y_{k+1}& \cdots & y_{k+N} \end{bmatrix}^T \hspace{-7pt}\in \mathbb{R}^{Np}$ could lie in a high dimensional plane than $\psi_o$ as $Np\geq n_o$
\end{itemize}
 Hence, we construct a diffeomorphic map between $\psi_o(x)$ and the projected time-delay embedded outputs $z_k \hspace{-2pt}=\hspace{-2pt} \mathcal{O}^T\hspace{-2pt}\begin{bmatrix} y_k & y_{k+1}& \cdots & y_{k+N} \end{bmatrix}^T \hspace{-4pt}=\hspace{-2pt} \mathcal{O}^T\mathcal{O}\psi_o(x_k) \hspace{-2pt}\in\hspace{-2pt} \mathbb{R}^{n_o}$. We explore the KO-based sensor fusion for the two dynamics in the following corollary. 

\begin{cor}
The dynamics of the projected time-delay embedded output $z$ is $   z_{k+1} =  \mathcal{O}^T\mathcal{O}K_o (\mathcal{O}^T\mathcal{O})^{-1}z_k$. We see that the dynamics of $z$ and $x$ are diffeomorphic conjugate under the map $z = H(x) = \mathcal{O}^T\mathcal{O}\psi_o(x),H:\mathbb{R}^{n_o} \rightarrow \mathbb{R}^{n_o}$. Hence, all eigenfunctions of $z$  can be mapped to the corresponding eigenfunctions in  $\psi_o(x)$.
\hspace*{\fill}~\qed\par
\end{cor}

% \begin{cor}
% For the time-delay embedded output, 
% \[
% z_k = 
% \begin{bmatrix}
% y_k\\
% y_{k+1}\\
% \vdots\\
% y_{k+N}
% \end{bmatrix}= 
% \begin{bmatrix}
% h(x)\\
% h \circ F_1(x)\\
% \vdots\\
% h \circ F_N(x)
% \end{bmatrix} = \mathcal{O}\psi_o(x_k)
% \]
% where the dynamics of the new variable $z$ is given by
% \begin{align*}
%     z_{k+1} &= \mathcal{O}\psi_o(x_{k+1}) \\
%     &= \mathcal{O}K_o\psi_o(x_{k}) \\
%     &=  \mathcal{O}K_o (\mathcal{O}^T\mathcal{O})^{-1}\mathcal{O}^Tz_k
% \end{align*}
% \textbf{Establishing the conjugacy map}
% We consider the two dynamics 
% \begin{align*}
%     x_{k+1} &= f(x_k), f:\mathcal{M} \rightarrow \mathcal{M}\\
%     z_{k+1} &= g(z_k), g:\mathbb{R}^{Np} \rightarrow \mathbb{R}^{Np}
% \end{align*}
% where $g(z_k) = \mathcal{O}K_o (\mathcal{O}^T\mathcal{O})^{-1}\mathcal{O}^Tz_k$ and the map between them is given by $z = H(x) = \mathcal{O}\psi_o(x),H:\mathcal{M} \rightarrow \mathbb{R}^{Np}$, we can see that the two dynamical systems are factor conjugate as
% \begin{align*}
%     H \circ f(x_k) &= H(x_{k+1}) = \mathcal{O}\psi_o(x_{k+1})\\
%     g \circ H(x_k) &= g(\mathcal{O}\psi_o(x_k)) \\
%     &= \mathcal{O}K_o (\mathcal{O}^T\mathcal{O})^{-1}\mathcal{O}^T\mathcal{O}\psi_o(x_k)\\
%     &= \mathcal{O}K_o\psi_o(x_k) = \mathcal{O}\psi_o(x_{k+1})\\
%     \Rightarrow  H \circ f(x) &= g \circ H(x)
% \end{align*}
% Suppose the eigendecomposition of $K_o = V_o\Lambda_o V_o^{-1}$, then the modal decomposition of the dynamics in $z$ yields
% \begin{align*}
%      z_{k+1} &= \mathcal{O}K_o (\mathcal{O}^T\mathcal{O})^{-1}\mathcal{O}^Tz_k\\
%     &=\mathcal{O}V_o\Lambda_o (V_o^{-1} (\mathcal{O}^T\mathcal{O})^{-1}\mathcal{O}^Tz_k)
% \end{align*}
% where $\phi_z(z_k) =V_o^{-1} (\mathcal{O}^T\mathcal{O})^{-1}\mathcal{O}^Tz_k$ are the eigenfunctions. Then, the corresponding eigenfunctions in the dynamics of $x$ is given by
% \begin{align*}
%      \phi_{xo}(x_k) &= \phi_z \circ H (x_k) = \phi_z(\mathcal{O}\psi_o(x_k))\\
%      &= V_o^{-1} (\mathcal{O}^T\mathcal{O})^{-1}\mathcal{O}^T\mathcal{O}\psi_o(x_k) = V_o^{-1}\psi_o(x_k)
% \end{align*}
% which are the eigenfunctions of $\psi(x_{k+1}) = K_o\psi(x_k)$. Hence, the eigenfunctions that get mapped between the 
% \end{cor}


We see that the OC-KO architecture can fuse the state and output dynamics even if the outputs do not capture the entire state dynamics. The above analysis shows that the OC-KO structure is such that the lifting functions capture the dynamics of the time-delay embedded outputs. This is an implicit constraint in the model structure of OC-KO. We explicitly show that the output dynamics constrain the OC-KO learning problem.

==> theorems/theorem_1_old_redundant.tex <==
\begin{thm}\label{theorem: outputs span all lifting functions}
 Given a nonlinear system (\ref{eq: nonlinear system with output}) with Koopman operator representation of the form (\ref{eq: Koopman system with output}).  Suppose $\psi(x)$ is a Koopman observable function, not necessarily state-inclusive.    Further, suppose that $h_1(x),..,.h_p(x)$ are linearly independent measurement functions of $x$.   Then the following statements are true. 
%such that each output function in $\{h_i:\mathcal{M} \rightarrow \mathbb{R}|i= 1,2,...p\}$ lies in the span of the Koopman operator lifting functions $\{\psi_i:\mathcal{M} \rightarrow \mathbb{R}|i = 1,2,...n_L\}$ which need not necessarily be state-inclusive, 
\begin{enumerate}
    \item if $\quad rank(W_h)=n_L$, then each scalar Koopman observable function $\psi_i(x)$ is uniquely determined by a mapping on $h(x)$ %\{h_1,...,h_p \}$ $\quad \forall \quad i \in\{1,2,...n \} $ 
    \item if $\quad rank(W_h)=r<n_L$, then there exists a transformed Koopman observable $\tilde{\psi}$, and corresponding similarity transformation $T$,  such that $r$ components of the vector Koopman observable $\tilde{\psi}(x)$ given by $\psi_h(x)$ are determined by a mapping on $h(x).$
    % $\psi_i \in span \{h_1,...,h_p \} \quad \forall \quad i \in\{1,2,...r \} $  
\end{enumerate}
\end{thm}

\begin{pf}
\textit{Case (1):} Since $W_h$ has full column rank, an exact left inverse exists such that 
\begin{align*}
    \psi(x_k) = (W_h^TW_h)^{-1}W_h^Th(x_k) \quad \forall \quad x_k \in \mathcal{M}
\end{align*}
and hence
$\psi_i \in span \{ h_1 , h_2, ..., h_p \}$ $\forall$ $i \in \{1,2,...,n_L\}$.\\
\textit{Case (2):} Suppose $rank(W_h) = r <n_L$. Since, it is given that outputs lie in the span of the lifting functions, $p \leq r$. The singular value decomposition of $W_h$ yields
\begin{align*}
W_h &= \begin{bmatrix}
        U_r & U_{p-r}
        \end{bmatrix}_{p\times p}
        \begin{bmatrix}
        \Sigma_r & 0\\
        0 & 0
        \end{bmatrix}_{p\times n_L}
        \begin{bmatrix}
        V_r^T\\ 
        V_{n_L-r}^T
        \end{bmatrix}_{n_L \times n_L}\\
%where $U_r$ and $U_{p-r}$ denote the first $r$ and the last $p-r$ left eigen vectors of $W_h^TW_h$, $V_r$ and $V_{n_L-r}$ denote the first $r$ and the last $n_L-r$ right eigen vectors of $W_h^TW_h$ and $\Sigma_r$ denote the $r$ eigenvalues of $W_h^TW_h$ that are nonzero.
\Rightarrow
    h(x_k) &= \begin{bmatrix}
        W_{h\psi} & 0
        \end{bmatrix}
        \begin{bmatrix}
        \psi_h(x_k)\\ 
        \bar{\psi}_{h}(x_k)
        \end{bmatrix} \quad \forall \quad x_k \in \mathcal{M}
\end{align*}
where $W_{h\psi} = U_r\Sigma_r, \text{ } \psi_h(x) = V_r^T\psi(x) \text{ and } \bar{\psi}_{h}(x) = V_{n_L-r}^T\psi(x)$. $W_{h\psi}$ has a full column rank $r>p$ and hence
\[
\psi_h(x_k) = (W_{h\psi}^TW_{h\psi})^{-1}W_{h\psi}^Th(x_k) \quad \forall \quad x_k \in \mathcal{M}.
\]
Therefore, under a similarity transformation $T \hspace{-4pt}= \begin{bmatrix}V_r & V_{n_L-r}\end{bmatrix}$ such that $\Tilde{K} = T^TKT$, $\Tilde{\psi}(x) = T^T\psi(x)$, $\Tilde{W}_h = W_hT$, (\ref{eq: Koopman system with output}) becomes
\begin{align*}
    \Tilde{\psi}(x_{k+1}) &= \Tilde{K}\Tilde{\psi}(x_k)\\ %\quad \backslash \quad
    y_k &= \Tilde{W}_h\Tilde{\psi}(x_k)
\end{align*}
where $\Tilde{\psi} = [\psi_h^T \quad \bar{\psi}_h^T]^T$ with the first $r$ lifting functions of $\Tilde{\psi}$ given by $\psi_h$ lie in the span of $h$.
\hspace*{\fill}~\qed\par
\end{pf}

Koopman observables are generally nonunique; they have infinite solutions. 
We see from Theorem \ref{theorem: outputs span all lifting functions} that when the $W_h$ matrix is full column rank, the outputs can uniquely determine the space of Koopman observables. Hence, the output dynamics can be represented by the entire state dynamics. In the event that $n_L<p$, the map $y=W_h\psi(x)$ is a map from a low dimensional space $\psi(x) \in \mathbb{R}^{n_L}$ to a high dimensional space $y \in \mathbb{R}^{p}$. To ensure maximum sensor fusion, we project the outputs to the lower dimensional $\mathbb{R}^{n_L}$ space so that the state and projected output dynamics are diffeomorphic conjugate. We fuse the dynamics using the method in Section \ref{sec: Fusion using Koopman operators}.

\begin{cor} \label{corollary: outputs form Koopman operator}
If $rank(W_h)=n_L<p$, we can construct a diffeomorphic map between the states and outputs by considering the projection $z= W_h^Ty$. The projected dynamics  $z_{k+1}= W_h^TW_hK(W_h^TW_h)^{-1}z_k$ has a diffeomorphic map $z = H(\psi(x)) = W_h^TW_h\psi(x), H:\mathbb{R}^{n_L}\rightarrow\mathbb{R}^{n_L}$ between $z$ and $\psi(x)$. Suppose, the modal decomposition (\ref{eq: modal decomposition practical}) of $z$ dynamics yields the eigenfunctions  $\phi_z(z) = (W_h^TW_h)^{-1}V^{-1}z_k$ where $K=V\Lambda V^{-1}$. The $\phi_z(z)$ can be mapped to the eigenfunctions of $\psi(x_{k+1}) = K\psi(x_k)$ by using (\ref{eq: sensor fusion KO eigenfunction map}):
$
\phi_{\psi}(\psi(x)) = \phi_z \circ H(\psi(x)) = V^{-1}\psi(x) 
$. The reverse map is given by $\phi_z(z) = \phi_{\psi} \circ H^{-1}(z)$ where $H^{-1}(z) = (W_h^TW_h)^{-1}z.$
\hspace*{\fill}~\qed\par
\end{cor}

The KO of the projected output $z$ and the OC-KO of the lifted state $\psi(x)$ are diffeomorphic conjugate with a bijective map between their eigenfunctions. In the event that $rank(W_h) = n_L =p$, the total output has a direct diffeomorphic map with $\psi(x)$.

\begin{cor}\label{cor: rank(W_h) = n_L =p}
For $rank(W_h) = n_L =p$, $W_h$ becomes an invertible square matrix and the output equation simplifies to $y_{k+1} = g(y_k)=W_hKW_h^{-1}y_k$ with all the eigenfunctions of the state dynamics $\phi_x(x) = V^{-1}\psi(x) $ mapping to the eigenfunctions of the output dynamics $\phi_y(x) = V^{-1}W_h^{-1}\psi(x) $ and vice versa.
\hspace*{\fill}~\qed\par
\end{cor}


% \begin{cor} \label{corollary: square W_h outputs form Koopman operator}
% If $rank(W_h)=n_L=p$, then there exists a bijective map between $h(x) \in \mathbb{R}^p$ and $\psi(x) \in \mathbb{R}^{n_L}$ as $h(x) = W_h\psi(x)$ and $\psi(x) = W_h^{-1}h(x)$. It follows that
% \begin{align}\label{eq: cor3 _1}
%     h(x_{k+1}) &= W_hKW_h^{-1}h(x_k)\nonumber\\
%     y_k &= \mathbb{I}h(x_k)
% \end{align}
% where $\mathbb{I}$ is the identity matrix can also represent the dynamics of (\ref{eq: nonlinear system with output}).
% Following the approach in Corollary \ref{corollary: outputs form Koopman operator}, we can say that the eigenfunctions of (\ref{eq: cor3 _1}) and (\ref{eq: Koopman system with output}) can be mapped using the $W_h$ matrix transformation. 
% \end{cor}
% \begin{cor} \label{corollary: outputs form Koopman operator}
% If $rank(W_h)=n_L=p$, then there exists a bijective map between $h(x) \in \mathbb{R}^p$ and $\psi(x) \in \mathbb{R}^{n_L}$ as $h(x) = W_h\psi(x)$ and $\psi(x) = W_h^{-1}h(x)$. It follows that
% \begin{equation}\label{eq: cor3 _1}
%     h(x_{k+1}) = W_hKW_h^{-1}h(x_k).
% \end{equation}
% Since there exist functions $F_1(\psi(x)) = K\psi(x),F_1:\mathbb{R}^{n_L} \rightarrow \mathbb{R}^{n_L}$ and $F_2(h(x)) = W_hKW_h^{-1}h(x),F_2:\mathbb{R}^{p} \rightarrow \mathbb{R}^{p}$ 
% and a map $G(\psi(x)) = W_h\psi(x) = h(x)$ such that $G\circ F_1 (\psi(x)) = F_2 \circ G(\psi(x))$, $h(x)$ and $\psi(x)$ are said to have a
% a topological conjugate map. If the eigen decompositon of $K$ is given by $K= V\Lambda V^{-1}$, then $\Phi_h(h(x)) = V^{-1}W_h^{-1}h(x)$ and $\Phi_\psi(\psi(x)) = V^{-1}\psi(x)$ are the eigenfunctions of (\ref{eq: cor3 _1}) and (\ref{eq: Koopman system with output}) respectively such that
% \begin{align*}
%     \Phi_h(h(x)) &= V^{-1}W_h^{-1}h(x)\\
%     \Phi_\psi(\psi(x)) =\Phi_h \circ G (\psi(x)) &= V^{-1}W_h^{-1}h(x).
% \end{align*}
% This is a subcase of Proposition 4.1 proved by Mezic \cite{mezic2019spectrum}.
% \end{cor}

==> theorems/theorem_K_OL,h_subseteq_K_OL.tex <==

\begin{thm} \label{theorem: K_OLh subset of K_OL}
Given the nonlinear system (\ref{eq: nonlinear system with output}), if $\mathcal{K}_{OL}$ and $\mathcal{K}_{OL,h}$ denote the set of all KOs consistent with (\ref{eq: NL_sys_without_output}) and (\ref{eq: nonlinear system with output}) respectively, then $\mathcal{K}_{OL,h} \subseteq \mathcal{K}_{OL}$.
%under finite output measurement and $\mathcal{K}_{OL,h} = \mathcal{K}_{OL}$ only for the trivial case $f(x_k) = 0$.
\end{thm}
\begin{pf}
Any KO that satisfies (\ref{eq: nonlinear system with output}) also captures (\ref{eq: NL_sys_without_output}). Hence, $\mathcal{K}_{OL,h} \subset \mathcal{K}_{OL}$ is always true. The condition $\mathcal{K}_{OL} = \mathcal{K}_{OL,h}$ is satisfied when all the eigenfunctions of the KO that capture the state dynamics can be mapped to the eigenfunctions  of the KO that constitute the output dynamics. This is seen in Corollary \ref{cor: rank(W_h) = n_L =p}. The condition $\mathcal{K}_{OL} \not\subset \mathcal{K}_{OL,h}$ follows from the previous cases. We prove it by contradiction by assuming $\mathcal{K}_{OL} \subset \mathcal{K}_{OL,h}$ is true. But we have already shown that $\mathcal{K}_{OL,h} \subset \mathcal{K}_{OL}$ is always true and hence the best case scenario is $\mathcal{K}_{OL,h} =\mathcal{K}_{OL}$.
\hspace*{\fill}~\qed\par
\end{pf}
